Putting Things into Context: Rich Explanations for Query Answers using Join Graphs (extended version)

In many data analysis applications, there is a need to explain why a surprising or interesting result was produced by a query. Previous approaches to explaining results have directly or indirectly used data provenance (input tuples contributing to the result(s) of interest), which is limited by the fact that relevant information for explaining an answer may not be fully contained in the provenance. We propose a new approach for explaining query results by augmenting provenance with information from other related tables in the database. We develop a suite of optimization techniques, and demonstrate experimentally using real datasets and through a user study that our approach produces meaningful results by efficiently navigating the large search space of possible explanations.

==> sections/algo-pattern-saved.tex <==
% \section{Summarization Algorithms}
% \label{sec:algo}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Mining Patterns given a Join Graph}
\label{sec:algo_pattern}

\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]\caption{{\bf \algMineAPT to find top-$k$ patterns given a join graph $\jgraph$}\\
{\bf Other inputs:} Database $D$, Query $Q$, Answer tuples in user question $t_1, t_2$,  limit on the number of categorical attributes in the pattern $\maptKcat$, and input parameters $\lambda$s described in text. }\label{alg:basic-pattern-mine}

  {\small
    \begin{codebox}
      \Procname{\proc{\algMineAPT} ($\db, \jgraph, \query, \tup_1, \tup_2, k, \maptKcat, \revc{\paramAfilterrate}$)}
      \li $\explset \gets \emptyset$ \Comment{min-heap: to store top-$\topk$ explanations by their score}
      \li $\maptAPT \gets \jtr({\jgraph, \db})$
      \li $\maptSample \gets \Call{createSample}{\maptAPT}$ \label{alg-line:mapt-sample}
      \li $(\maptAnum, \maptAcat, \maptCluster) \gets \Call{\maptFilterAttrs}{\maptAPT, \revc{\paramAfilterrate}}$
      \li $\patLCA \gets \Call{LCA}{\maptSample, A_{cat}}$ \label{alg-line:mapt-lca} \Comment{from \cite{DBLP:journals/pvldb/GebalyAGKS14}}
      \li $\maptTODO \gets \Call{pickTopK}{\patLCA,\maptKcat,\maptAPT}$ \label{alg-line:cat-top-k}
      \li $\maptDONE \gets \emptyset$
      \li \While $\maptTODO \neq \emptyset$ \label{alg-line:mapt-refine}
         \Do
         \li $\maptPat \gets \Call{pop}{todo}$
         \li $\maptDONE \gets \maptDONE \cup \{ \maptPat \}$
         \li \For $\tup_{cur} \in \{ \tup_1, \tup_2 \}$ \Do
             \li \If $\Call{recall}{\maptPat,\tup_{cur}} > \paramRecallThresh$ \label{alg-line:mapt-filter-recall}\Then
                 \li \If $\Call{F1}{\maptPat,\tup_{cur}} > \Call{F1}{\textsc{peek}(\explset)}$ \Then
                     \li $\explset \gets \Call{deleteMin}{\explset}$
                     \li $\explset \gets \Call{insert}{\explset, (\maptPat, \tup_{cur})}$
                     \End
                 \li \For $A \in \maptAnum$ \Do
                     \li \If $\maptPat.A = \placeh$ \Then
                         \li \For $op \in \{=, \leq\}, c \in \Call{getFragments}{\domOf{APT}{A}}$ \Do
                              \li $\maptPatnew \gets \maptPat$
                              \li $\maptPatnew.A \gets \patop{op}{c}$
                              \li \If $\maptPatnew \not\in done$ \Then
                                  \li $\maptTODO \gets \maptTODO \cup \{ \maptPatnew \}$
                              \End
                         \End
                      \End
                  \End
             \End
          \End
      \End
    \li \Return $\explset$
    \end{codebox}
    \begin{codebox}
      \Procname{$\proc{\maptFilterAttrs}(\maptAPT, \paramAfilterrate)$}
      \li $A \gets \schemaOf{\maptAPT}$
      \li $\maptAfilter \gets \Call{filterBasedOnRelevance}{\maptAPT, \paramAfilterrate}$ \label{alg-line:mapt-filter-attrs-relevance}
      \li $\maptCluster \gets \Call{clusterAttributes}{\maptAfilter, \maptAPT}$ \label{alg-line:mapt-filter-attrs-cluster}
      \li $\maptArepresent \gets \Call{pickClusterRepresentatives}{\maptCluster, \maptAPT}$ \label{alg-line:mapt-filter-attrs-pick-representatives}
      \li $\maptAnum \gets \{ A \mid A \in \maptArepresent \land A \mathtext{is numeric} \}$
      \li $\maptAcat \gets \{ A \mid A \in \maptArepresent \land A \mathtext{is categorical} \}$
      \li \Return $(\maptAnum, \maptAcat, \maptCluster)$
    \end{codebox}
    }
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we present our algorithm (\Cref{alg:basic-pattern-mine}) for mining patterns from an augmented provenance table
(\abbrAPT) $\jtr(Q, \db, \jgraph)$ generated based on a given join graph $\jgraph$. Recall that we are dealing with patterns that may contain
equality comparisons (for categorical attributes) and/or inequality comparisons (for numeric attributes). %Inequality comparisons are only considered for numerical attributes.
We mine patterns in multiple
phases. (i) In a preprocessing step (\Cref{alg:basic-pattern-mine}, function \proc{\maptFilterAttrs}), we use random forests to determine the
relevance of each attribute on predicting tuples to belong to the provenance of
one of the two data points from the user's question. The purpose of this step is to remove attributes that
are unlikely to yield patterns of high quality. Then we cluster attributes that
are highly correlated to reduce redundancy in the generated patterns. The
output of this preprocessing step are the generated clusters and one
representative selected for each cluster.  (ii) In the next phase of pattern mining (line~\ref{alg-line:mapt-lca} and following)
we only consider categorical attributes and mine pattern candidates using a
variation of the \emph{LCA (Least Common Ancestor)} method from~\cite{DBLP:journals/pvldb/GebalyAGKS14} that can only handle categorical attributes. From the set of patterns returned by the LCA method, we then select the  $\maptKcat$ patterns with the highest scores for the next step (line~\ref{alg-line:cat-top-k}).
%\red{CHECK} %\red{Add the full form of LCA and a line on the summary of this method.} (iii) From the set of patterns generated in this fashion we then select a subset of further consideration \red{HOW??}.
(iii) These patterns are then \emph{refined} (line~\ref{alg-line:mapt-refine} and following) by adding conditions on
numerical attributes that can improve precision at the potential cost of
reducing recall. (iv) The refined patterns are filtered to remove patterns with
recall below a threshold $\paramRecallThresh$ (line~\ref{alg-line:mapt-filter-recall}) and are ranked by their score according
to~\Cref{def:metrics}. Finally, the top-k patterns according to this
ranking are returned. % The full algorithm is shown
% in~\Cref{alg:basic-pattern-mine}.

Before describing the individual steps of our pattern mining algorithm, we first
need to introduce additional notation used in this section. Given a pattern
$\pat$, we call a pattern $\pat'$ a {\bf refinement} of $\pat$ and $\pat'$ can
be derived from $\pat$ by replacing one or more placeholders ($\placeh$) with
comparisons. For instance, pattern $\pat_2 = (\peq{X}, \pleq{Y})$ is a
refinement of $\pat_1 = (\peq{X}, \placeh)$.
%\BG{Adapt if we do not get to  that.}
The following observation holds:
  \begin{proposition}
  Using Definition~\ref{def:metrics}, given a tuple $t \in Q(D)$ and a join graph $\jgraph$, $\Rec(\sexpl_2, \jgraph,  \tup)
\leq \Rec(\sexpl_1, \jgraph,  \tup)$, where $\sexpl_1 = (\jgraph, \pat_1)$, $\sexpl_2 = (\jgraph, \pat_2)$, and $\pat_2$ is a refinement of $\pat_1$.
  \end{proposition}
  \begin{proof}
  Following Definition~\ref{def:metrics} (a), if a $\tup' \in \pt{\query, \db, \tup}$ is covered by $\sexpl_2$, then it is also covered by $\sexpl_1$. Hence, by (b) and (d),  $\ITP(\sexpl_1, \jgraph, \tup) \geq \ITP(\sexpl_2, \jgraph, \tup)$ and $\IFN(\sexpl_1, \jgraph, \tup) \leq \IFN(\sexpl_2, \jgraph, \tup)$. Therefore, using (e), $\Rec(\sexpl_2, \jgraph,  \tup)
\leq \Rec(\sexpl_1, \jgraph,  \tup)$.
  \end{proof}
 % Since if a tuple  that the recall of a refined pattern has to be less than or equal to the recall of the pattern it is derived from \red{NEED A PROPOSITION?}.
We exploit the above fact to
exclude patterns and their refinements early on in the process if their recall
is below a threshold.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Filtering and Clustering Attributes}
\label{sec:filt-clust-attr}

Before mining patterns, we analyze the attributes of an \abbrAPT to (1) determine the attributes that are unlikely to contribute to top-k patterns because they are not helpful in distinguishing between the two outputs of interested provided as part of the user's question, and (2) to identify clusters of attributes with strong mutual correlations, because such attributes can lead to redundancy in explanations as discussed below. The pseudo code for method $\proc{\maptFilterAttrs}$ implementing this step is shown in~\Cref{alg:basic-pattern-mine}. %\red{need to mention procedure names from the pseudocode to the corresponding method in text}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Filtering Attributes based on Relevance}
Random forests have been successfully used in machine learning applications  to determine the relevance of a feature (attribute) to the outcome of a classification task.
We train a random forest  classifier (line~\ref{alg-line:mapt-filter-attrs-relevance}) that predicts whether a row belongs to the augmented provenance of one of the two outputs from the user's question~\cite{breiman2001random}. %\BG{Cite some work that discusses using random forests to rank features}
We then rank attributes based on the relevance and find the fraction $\paramAfilterrate$ of attributes with the highest relevance ($\paramAfilterrate$ is a threshold used by the system).
The rationale for this step is to avoid generating patterns involving attributes that are irrelevant for distinguishing the two output tuples $t_1, t_2$ in the user question. This reduces the search space for patterns and additionally has the advantage of excluding attributes that are mostly constant in the rows contributing to the two outputs. Such attributes can be added to any pattern with minimal effect on the recall and precision of patterns, since they essentially do not affect the matches for the patterns. This could mislead users into thinking that the value of this attribute is a distinguishing factor for the tuples in the user question when in fact the value of this attribute has very limited or no effect.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Clustering Attributes based on Correlations}
Additional redundancy in patterns can be caused by attributes that are highly correlated. As an extreme example, consider an \abbrAPT containing both the birth date and age of a person. For any pattern containing a predicate on birth date there will be an (almost) equivalent pattern using age instead and a pattern restricting  both age and birth date. To reduce the prevalence of such redundant patterns, we cluster attributes based on their mutual correlation (line~\ref{alg-line:mapt-filter-attrs-cluster}) and pick a single representative for each cluster (line~\ref{alg-line:mapt-filter-attrs-pick-representatives}). We use VARCLUS~\cite{sarle1990sas}, a clustering algorithm closely related to principal component analysis and other dimensionality reduction techniques~\cite{roweis2000nonlinear}. However, any technique that can cluster correlated attributes would be applicable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{%Generating
Patterns over Categorical Attributes}
\label{sec:gener-patt-over}

We then generate a sample of size $\paramPatsamplerate$ (an input parameter) from %\abbrAPT
$\jtr(Q, \db, \jgraph)$ (line~\ref{alg-line:mapt-sample}) and
generate a set of candidate patterns over categorical attributes (ignoring all
numerical attributes at this stage) using the LCA method
from~\cite{DBLP:journals/pvldb/GebalyAGKS14} (line~\ref{alg-line:mapt-lca}).  The LCA method generates pattern
candidates from a sample by computing the cross product of the sample with
itself.
%\red{not clear -- need a few more lines on LCA method}.
A candidate pattern is generated for each pair $(t,t')$ of tuples from
the sample by replacing values of attributes $A$ where $t.A \neq t'.A$ with a
placeholder $\placeh$ and by keeping constants that $t$ and $t'$ agree upon
($t.A = t'.A$). Note that in our case each element of a pattern is a
predicate. Thus, using a constant as done in the LCA method corresponds to using
an equality predicate, i.e., $A = c$ for $t.A = t'.A = c$. By keeping constants
that frequently co-occur, the LCA method that only
works for categorical attributes (equality comparisons) generates patterns that reflect common
combinations of constants in the data.  Note that we ignore numeric attributes
at this step, i.e., we use $\placeh$ for all numeric attributes.  The
rationale of focusing on categorical attributes first is that we can (i) use the
established heuristic of the LCA method to generate pattern candidates from categorical attributes, and (ii) we can
significantly reduce the search space by pruning all refinements of patterns
that fail to have a sufficiently high recall.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Filtering Categorical Pattern Candidates}
\label{sec:filt-categ-patt}

Next we calculate the recall for each pattern by filtering the input
table to determine the matches of the pattern. As an optimization, we can calculate the
recall over a sample of the data (using a sample size parameter
$\paramQualitysamplerate$). %Note that we use
This may require using a separate sample size ($\maptKcat$) since we found that a small sample is sufficient for generating a meaningful set of
patterns, but may not be sufficient for estimating recall with high enough
accuracy.
%\BG{In the implementation we use a sample rate plus some lower and upper bound on the sample size. Describe this here or keep it simple?}
Irrespective of whether the recall is estimated or calculated precisely, we then filter
out patterns whose recall is below a threshold $\paramRecallThresh$. Out of these
patterns, we then pick the top patterns based on their recall.
%\BG{We use frequency of the pattern in the LCA result in the implementation, what to do about that?}
In the following we use $\patLCA$ to denote the set of patterns
that are returned by this step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Refinement and Numeric Attributes}
\label{sec:pattern-refinement}
In the next step, we then generate refinements of patterns from $\patLCA$ by replacing placeholders on numerical attributes with predicates. Even though such refinements can at best have the same recall as the pattern they originate from, their precision may be higher resulting in greater \abbrFs. Recall that for numerical attributes we allow for both equality as well as inequality predicates. Domains of numerical attributes are typically large, resulting in large number of possible constants to use in inequality comparisons. To reduce the size of the search space, we split the domain of each numerical attribute into a fixed number $\paramNumRefineFrags$ of
%equally-sized
fragments (e.g., quartiles) and only use boundaries of these fragments when generating refinements. For example, for $\paramNumRefineFrags = 3$ we would use the minimum, median, and maximum value of an attribute's domain.
We systematically enumerate all refinements of a pattern by extending it by one predicate at a time. For each such refinement we calculate its recall as described above. Patterns whose recall is below $\paramRecallThresh$ are not further refined. We use $\patset_{refined}$ to denote the union of  $\patset_{LCA}$ with the set of patterns generated in this step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computing Top-k Patterns}
\label{sec:computing-top-k}

\newcommand{\wscore}{\textsc{wscore}}
\newcommand{\dscore}{\mathcal{D}}
\newcommand{\patres}{\mathcal{R}}
\newcommand{\dmatchs}{\textsc{matchscore}}

Finally, we calculate the \abbrFs for each pattern in $\patset_{refined}$ and return $k$ patterns.
\revm{To improve the diversity of the returned patterns we rank them based on a score that combines \abbrFs (\Cref{def:metrics}) with a diversity score $\dscore(\pat,\pat')$ that measure how similar two patterns are. The first pattern to be returned is always the one with the highest \abbrF. Then we determine the $i+1^{th}$ pattern based on this score. Note that the diversity score $\mathcal{D}(\pat)$ for a pattern $\pat$ depends on the set $\mathcal{R}$ of patterns we have selected to far, because it measure how close the pattern $\pat$ is to the most similar pattern in $\mathcal{R}$. We calculate this as a score $\dscore(\pat,\pat')$ that ranges between -2 and 1 (larger scores means that the two patterns are more dissimilar). The formula for calculating the score is shown below.  For each attribute $A$ of pattern $\pat$ we add 1 if the attribute does not appear in $\pat'$, we add a penalty (-0.3) if the attribute appears in both patterns (but with different constants), and a larger penalty (-2) if it appears in both patterns with the same constant. We repeatedly add the pattern with the highest score to $\mathcal{R}$ until we have $k$ patterns to return.} % include for each attribute $A$ of the pattern
% with the highest scores according to .
 % We use a min-heap to keep track of top-$k$ patterns, and replace the lowest of current top-$k$ if we encounter a higher \abbrF value.
\revm{
  \[ \wscore(\pat) = \fscore(\sexpl, \jgraph,  \tup_1, \tup_2) + \min_{\pat' \in \patres} \dscore(\pat,\pat') \]
  \[ \dscore(\pat,\pat') = \frac{\sum_{A: \pat.A \neq \placeh} \dmatchs(\pat,\pat',A) }{\card{\pat}}\]
  \[
    \dmatchs(\pat,\pat',A) =
    \begin{cases}
      1    & \pat'.A = \placeh        \\
      -0.3 & \pat.A[0] \neq \pat.A[0] \\
      -2   & \pat.A[0] \neq \pat.A[0] \\
    \end{cases}
  \]
}
We denote the result of this step as $\pattopk$.

\todoC{Describe our new diversity approach} To avoid repetitive attributes and values appear in the top-$k$ results, we implemented a pattern diversification approach, which would add penalties to the same attributes and same values that have appeared in the previous results within top-$k$ results.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/algo_graph_saved.tex <==
\section{Join Graph Enumeration}\label{sec:join-graph-enumeration}

  \newcommand{\jgZero}{\jgraph_0}
  \newcommand{\algjgJSize}{JSize}
  \newcommand{\algjgIsValid}{isValid}
  \newcommand{\algjgAddEdge}{AddEdge}
  \newcommand{\algjgGenNewJG}{ExtendJG}
  \newcommand{\algjgExpls}{\mathcal{E}}
  \newcommand{\algjgPK}{getPK}
  \newcommand{\algjgnone}{n_1}
  \newcommand{\algjgntwo}{n_2}
  \newcommand{\algjgRels}{rels}
  \newcommand{\algjgStart}{start}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}
  \caption{Join Graph Enumeration}\label{alg:join-graph-enumeration}
{\small
  \begin{codebox}
    \Procname{\proc{\JGGen}$(\jgZero, \asgraph, \query,k, k_{cat})$}
    \li $\algjgExpls \gets \emptyset$ \Comment{maps join graphs to explanations}
	\li $\jgraphs{} \gets \{\jgZero\}$ \Comment{generated join graphs}
	\li $\jgraphs{prev} \gets \{\jgZero\}$ \Comment{join graphs from the previous iteration}
	\li \While $\algjgJSize \in \{ 1, \ldots, \paramJoinGraphSize \}$ \label{alg-line:jge-main-loop}
	\li \Do $\jgraphs{new} \gets \emptyset$ \Comment{join graphs generated in this iteration}
	\li \For $\jgraph \in \jgraphs{prev}$ \Do
    \li $\jgraphs{new} \gets \jgraphs{new} \cup \proc{\algjgGenNewJG}(\jgraph,\asgraph, \query$)  \label{alg-line:jge-extend-jg}
    \End
        \li \For $\jgraph \in \jgraphs{new}$ \Do
    \li \If $\Call{\algjgIsValid}{\jgraph}$ \Then \label{alg-line:jge-test-valid}
    \li $\algjgExpls[\jgraph] \gets \Call{\algMineAPT}{\db, \jgraph, \query, t_1, t_2, k, k_{cat}}$
    \End
    \End
    \li $\jgraphs{} \gets \jgraphs{} \cup \jgraphs{new}$
    \li $\jgraphs{prev} = \jgraphs{new}$
    \End
    \li \Return $\algjgExpls$
      \end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      	\begin{codebox}
	\Procname{\proc{\algjgGenNewJG}($\asgraph, \jgraph, \query$)}
	\li $\jgraphs{new} \gets \emptyset$
	\li \For $v \in \jgraphnodes$ \Do
	\li \If $\tlabelv(v) = \ptlabel$ \Then
    \li $\algjgRels \gets \relsinQ$
    \li \Else
    \li $\algjgRels \gets \tlabelv(v)$
    \End
	\li  \For  $r \in \algjgRels, n \in \snodes{}$ \Do
       \li $e \gets (r,n)$
        	\li \If $e \in \sedges{}$ \Then \label{alg-line:extjg-iterate-edges}
        	\li \For  $c \in \sglabel(e)$ \Do
                \li $\jgraphs{new} \gets \jgraphs{new} \cup \Call{\algjgAddEdge}{\jgraph, v, n, c}$
                \End
                \End
                \End
    \End
    \li \Return $\jgraphs{new}$
  \end{codebox}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   	\begin{codebox}
   	\Procname{\proc{\algjgAddEdge}($\jgraph, v, end, cond$)}
   	\li $\jgraphs{added} \gets \emptyset$
    \li $\jgraph_{curr} \gets \jgraph$ \Comment{Add $end$ as new node}
    \li $v_{new} \gets \Call{newNode}{$\,$}, e \gets (v,v_{new})$
    \li $\jgraph_{curr}.\jgraphnodes \gets \jgraph_{curr}.\jgraphnodes \cup \{v_{new}\}$
    \li $\jgraph_{curr}.\tlabelv(v_{new}) \gets end$
    \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{e\}$
    \li $\jgraph_{curr}.\tlabele(e) \gets cond$
    \li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
    %%%%%%%%%%
   	\li \For $v' \in \jgraph.\jgraphnodes: \tlabelv(v') = end$ \Comment{Add edge connecting existing nodes} \Do
           	\li \If $\neg \exists e \in \jgraph.\jgraphedges: e = (v,v') \land \jgraph.\tlabele(e) = cond$ \Then
           	\li $\jgraph_{curr} \gets \jgraph$
            \li $e \gets (v,v')$
            \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{e\}$
            \li $\jgraph_{curr}.\tlabele(e) \gets cond$
           	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
        \End
             \End
    \li \Return $\jgraphs{added}$
   	\end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{codebox}
        \Procname{\proc{\algjgIsValid}$(\jgraph)$}
        \li \For $v \in \jgraphnodes$ \Do
        \li \For $A \in \Call{\algjgPK}{\tlabelv}$ \Do
        \li \If $\neg \exists e \in \jgraphedges: A \in \attrs(\tlabele(e))$ \Then
        \li \Return $\bfalse$
        \End
        \End
        \End
        \li \If $\Call{estimateCost}{\jgraph} > \paramMaxQcost$ \Then
        \li \Return $\bfalse$
        \End
        \li \Return $\btrue$
      \end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section,
%we present our algorithm for enumerating join graphs ($\algogbasic$). The
we describe an algorithm
%present \Cref{alg:join-graph-enumeration} 
that enumerates join graphs  of iteratively increasing size (details in full version).  In iteration $i$, we enumerate all join
graphs with $i$ edges by adding a single edge conforming to the schema graph to
one of the join graphs of size $i-1$ produced in the previous iteration. The
maximum size of join graphs considered by the algorithm is determined by
parameter \paramJoinGraphSize. We employ several heuristic tests to determine
whether a join graph generated by the algorithm should be considered for pattern
mining. The rationale for not considering all join graphs for pattern mining is
that pattern mining can be significantly more expensive than just generating a
join graph, so  %Thus, we have an incentive to
we skip pattern mining for join graphs
that are either unlikely to yield patterns of high quality or for which
generating the \abbrAPT and patterns are likely to be expensive.  For join
graphs that pass these tests we materialize the corresponding \abbrAPT and
apply the pattern mining algorithm from \Cref{sec:algo_pattern} to compute the
top-k patterns for the \abbrAPT.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generating Join Graphs}
\label{sec:gener-join-graphs}

We enumerate join graphs in iteration $i$ by extending every join graph produced in iteration $i-1$ with all possible edges. For each join graph $\jgraph$ produced in iteration $i-1$, we consider two types of extensions: (i) we add an additional edge between two existing nodes of the graph and (ii) we add a new node and connect it via a new edge to one of the existing nodes of the graph. The main entry point is function \textsc{\JGGen} from \Cref{alg:join-graph-enumeration}. We first initialize the result to contain $\jgZero$, the join graph consisting of a single node labeled ($\ptlabel$).
Within each iteration of the main loop (line~\ref{alg-line:jge-main-loop}), each join graph $\jgraph$ from the set of join graphs generated in the previous iteration ($\jgraphs{prev}$) is passed to function \proc{\algjgGenNewJG} which computes the set of all possible extensions of $\jgraph$ (line~\ref{alg-line:jge-extend-jg}). For any such join graph produced in this step, we then check whether it should be considered for patterning mining using function described below (line~\ref{alg-line:jge-test-valid}). For any join graph passing this check we call \proc{\algMineAPT} to generate the top-k patterns and store them in $\algjgExpls$.

% passing it along with the schema graph $\asgraph=\sgraph$ to \proc{\algjgGenNewJG}. \proc{\algjgGenNewJG} will add one more edge to the passed join graph (denoted as $\jgraph$) exhaustively by traversing each node in the $\jgraph$.

Function \proc{\algjgGenNewJG} enumerates all possible extension of a join graph with one additional edge. For that we consider all existing nodes $v$ in the join graph as possible extension points. We then enumerate all edges from the schema graph $\sgraph$ that are adjacent to nodes $r$ for relations that are represented by $v$. For that we have to distinguish two cases.  If $v$ is labeled $\ptlabel$, then $r$ can be any relation accessed by the query. Otherwise, there is a single node $r$ that is determined based on $v$'s label (the relation represented by $v$). For each edge $e$ adjacent to a node $r$ (line~\ref{alg-line:extjg-iterate-edges}), we then iterate over all conditions $c$ from the label of $e$ and then use function \proc{\algjgAddEdge} to enumerate all join graphs generated from $\jgraph$ by connecting $v$ with an edge labeled with $c$ to another node (either already in the join graph or new node added to the graph).

Function \proc{\algjgAddEdge} first generates a join graph by adding a new node $v_{new}$ labeled $end$ (the relation that is the end point of the edge in the schema graph) and connects it to $v$. Afterwards, for each node in the join graph $\jgraph$ labeled $end$ that is not connected to $v$ though an edge labeled $cond$ already, we generate a new join graph by adding such an edge.

% we consider two scenarios, one is if the node we are processing is $\ptlabel$ (line 3-10), then we will traverse $\relsinQ$ one by one. The other one is that the node is just one relation (line 11-17). Once \proc{\algjgGenNewJG} has found an valid edge to add (need to have 2 nodes $r,n$ and a condition on the edge $c$), it pass those arguments along with the $\jgraph$ being processed to \proc{\algjgAddEdge}. \proc{\algjgAddEdge} then try to first find the first node of the edge ($\tlabelv(v)==rel_1$) from $\jgraph$. Then \proc{\algjgAddEdge} traverse through $\jgraph$ see if there exists an node $\tlabelv(v')==rel_2$ and at the same time, $(v,v')$ does not exist in the edges of the $\jgraph$. If it is the case, \proc{\algjgAddEdge} will add this edge with the assignment of condition $cond$. Note in line 10-line 15 in \proc{\algjgAddEdge}, it will always add a new node $v''$ and new edge $(v,v'')$ to $\jgraph$.



% The \JGGen first starts by initializing the generated join graphs $\jgraphs{}$ as only having one join graph which only has one node contains $\ptlabel$. $\jgraphs{prev}$ denotes the generated join graph set from the previous iteration, initialized also only contains one same join graph as in $\jgraphs{}$. Then the algorithm iterates until the maximum number of operations allowed N is reached.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Checking Join Graph Connectivity and Skipping Expensive \abbrAPT Computations}
\label{sec:checking-join-graph}

We use the function \proc{\algjgIsValid} shown in~\Cref{alg:join-graph-enumeration}
to filter out join graphs based on lack of connectivity (described in the
following) or based on high estimated computation costs.

Note that schema graphs may contain tables with multiple primary key attributes
that are connected to edges which join on part of the key. This is typical in
``mapping'' tables that represent relationships. For instance, consider the
{\tt PlayerGameScoring} table from our running example that stores the number
of points a player scored in a particular game. Assume that there exists another
table player that is not part of the running example.  The primary key of this
table consists of a foreign key to the game table and the name of the player for
which we are recording stats. For this current example also assume that the
schema graph permits that {\tt PlayerGameScoring} to be joined with the {\tt Player} table.
Consider a query that joins the {\tt Game} table with {\tt LineupPerGameState},
{\tt LineupPlayer}, and {\tt Games} tables and selects games played by team GSW. A valid
join graph for this query would be to join the node $\ptlabel$ with
{\tt PlayerGameScoring} on the primary key of game. Note that while the result of the
query contains rows that pair a player of GSW with one lineup they played in a
particular game, the \abbrAPT would pair each row with any player that played in
that game irrespective of their team. Join graphs like this can lead to
redundancy and large \abbrAPT tables. One reason for this redundancy is that not
all primary key attributes of the {\tt PlayerGameScoring} table are joined with
another table. To prevent such join graphs that because of their redundancy
often lead to large \abbrAPT tables, function \proc{\algjgIsValid} checks that
for every node in the join graph, the primary key attributes of the relation
corresponding to that node are joined with at least one other node from the join
graph. For instance, in the example above the join graph could be modified to
pass this check by also joining the {\tt PlayerGameScoring} table with the Player
table.

Even though we filter join graphs that are not fully connected, some generated
join graphs will result in \revc{\abbrAPT}s of significant size which are expensive to
materialize and have significantly high cost for pattern mining. Recall that we
use queries to materialize join graphs.  We use the DBMS to estimate the cost of this query upfront. We
skip pattern mining for join graphs where the estimated cost of this query is
above a threshold $\paramMaxQcost$. While we may lose explanations by skipping
such join graphs, experimental results demonstrate that it is necessary for
reasonable performance to apply this check. \reva{Further, 
%a limitation of join graph size is not unreasonable, %because a user has to comprehend both the pattern as well as the join graph to understand an explanation. Thus, 
keeping the join graph size relatively small is likely not to overload the user with too complex explanations.
}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Skipping Expensive \abbrAPT Computations}
% \label{sec:skipp-expens-abbr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ranking Results}
\label{sec:ranking-results}

\revc{After we have enumerated join graphs and have computed top-k patterns for each join graph, we rank the union of all the pattern sets based on their \abbrF. We decided to rank patterns rather than filter patterns to reduce the load on the user by increasing the likelihood that good patterns are shown early, but without having the risk of completely filtering out patterns that have lower scores.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Computing \abbrAPTs}
% \label{sec:computing-abbrapts}



% \BG{OLD:}
% It takes 4 parameters as input. the schema graph $\asgraph$, a join graph $\jgraph_0$ which only has one node labeled as $\ptlabel$, the maximum number of operations allowed N when constructing a join graph from $\ptlabel$, and the set of relations accessed by query $\relsinQ$. Note here we define an ``operation'' as either adding an edge along with a new node if this node from the edge does not exist in the current join graph, or adding an edge without adding a new node.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{\algogbasic}
% {\small
% 	\begin{codebox}
% 	\Procname{\JGGen($\jgraph_0$, $\asgraph$, $\relsinQ$,N)}
% 	\li $\jgraphs{}$ $\gets \{\jgraph_0\}$ \Comment{generated join graphs}
% 	\li $\jgraphs{prev} \gets$ \{$\jgraph_0$\} \Comment{Initialize previous step set}
% 	\li JSize $\gets 1$
% 	\li \While JSize $\leq N$
% 	\li \Do $\jgraphs{new} \gets \emptyset$ \Comment{new join graphs we get in this iteration}
% 	\li \For $\jgraph$ in $\jgraphs{prev}$
%         \li \Do  $\jgraphs{new} \gets \jgraphs{new} \cup$ \proc{\algjgGenNewJG}($\jgraph,\asgraph, \relsinQ$)
%             \End
%             \li $\jgraphs{} \gets \jgraphs{} \cup \jgraphs{new}$
%             \li $\jgraphs{prev} = \jgraphs{new}$
%             \li JSize  $\gets$ JSize + 1
%         \End
%         \li \Return $\jgraphs{}$
%       \end{codebox}
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	\begin{codebox}
% 	\Procname{\proc{\algjgGenNewJG}($\asgraph, \jgraph, \relsinQ$)}
% 	\li $\jgraphs{new} \gets \emptyset$
% 	\li \For $v \in \jgraph.\jgraphnodes$
% 	\li \Do \If $\tlabelv(v) == \ptlabel$
% 	\li \Then \For  $r \in \relsinQ$
%         \li \Do \For  $n \in \asgraph.\snodes{}$
%         	\li \Do \If (($r, n) \in \asgraph.\sedges{}$)
%         	\li \Then \For  $c \in \sglabel((r, n))$
%             \li \Do $\tlabele((r,n))=c$
%             \li $\jgraphs{added} \gets $\proc{\algjgAddEdge}($\jgraph, \ptlabel, n, c$)
%             \li $\jgraphs{new} \gets \jgraphs{new} \cup \jgraphs{added} $
%                 \End
%             \End
%         \End
%     \End
%     \li \Else $r \gets \tlabelv(v)$
%     \li \For $n \in \asgraph.\snodes{}$
%     \li \Do \If (($r, n) \in \asgraph.\sedges{}$)
%     \li \Then \For  $c \in \sglabel((r, n))$
%     \li \Do $\tlabele((r,n))=c$
%     \li $\jgraphs{added} \gets $\proc{\algjgAddEdge}($\jgraph, r, n, c$)
%     \li $\jgraphs{new} \gets \jgraphs{new} \cup \jgraphs{added} $
%                 \End
%             \End
%         \End
%     \End
%     \End
%     \li \Return $\jgraphs{new}$
%   \end{codebox}
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    	\begin{codebox}
%    	\Procname{\proc{\algjgAddEdge}($\jgraph, rel_1, rel_2, cond$)}
%    	\li $\jgraphs{added} \gets \emptyset$
%    	\li \For $v \in \jgraph.\jgraphnodes$
%        	\li \Do \If $\tlabelv(v) == rel_1$
%            	\li \Then \For $v' \in \jgraph.\jgraphnodes$
%            	\Comment{\tiny Loop throught existing nodes see if $rel_2$ already exists in $\jgraph$}
%            	\li \Do \If $\tlabelv(v') == rel_2$ {\bf and} $(v,v') \notin \jgraph.\jgraphedges$
%            	\li \Then $\jgraph_{curr} \gets \jgraph$
%            	\li $\tlabele((v,v')) \gets cond$
%            	\li $\jgraph_{curr}.\jgraphedges \cup \{(v,v')\}$
%            	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
%     \End
%         \End
%        	\li $\jgraph_{curr} \gets \jgraph$
%         \Comment{\tiny No matter if this edge exist already, add a new edge with ($rel_1, rel_2$) here}
%         \li $v'' \gets \tlabelv^{-1}(rel_2)$
%         \li $\jgraph_{curr}.\jgraphnodes \gets \jgraph_{curr}.\jgraphnodes \cup \{v''\}$
%         \li $\tlabele((v,v')) \gets cond$
%         \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{(v, v'')\}$
%        	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
%             \End
%                \End
%     \li \Return $\jgraphs{added}$
%    	\end{codebox}
% }
% \end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/algo_merged.tex <==


\section{Algorithms for Mining Patterns}
\label{sec:algo}
In this section we discuss our algorithms for mining patterns for a given join graph (\Cref{sec:algo_pattern}), and for
enumerating all join graphs over which patterns should be mined (\Cref{sec:join-graph-enumeration}). \revm{Pseudocode for these algorithms and additional details are presented in \cite{chenjie2021}.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-5mm}
% \section{Mining Patterns given a Join Graph}
\subsection{Mining Patterns given a Join Graph}
\label{sec:algo_pattern}

\iftechreport{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]\caption{{\bf \algMineAPT to find top-$k$ patterns given a join graph $\jgraph$}\\
{\bf Other inputs:} Database $D$, Query $Q$, Answer tuples in user question $t_1, t_2$,  limit on the number of categorical attributes in the pattern $\maptKcat$, and input parameters $\lambda$s described in text. }\label{alg:basic-pattern-mine}

  {\small
    \begin{codebox}
      \Procname{\proc{\algMineAPT} ($\db, \jgraph, \query, \tup_1, \tup_2, k, \maptKcat, \revc{\paramAfilterrate}$)}
      \li $\explset \gets \emptyset$ \Comment{min-heap: to store top-$\topk$ explanations by their score}
      \li $\maptAPT \gets \jtr({\jgraph, \db})$
      \li $\maptSample \gets \Call{createSample}{\maptAPT}$ \label{alg-line:mapt-sample}
      \li $(\maptAnum, \maptAcat, \maptCluster) \gets \Call{\maptFilterAttrs}{\maptAPT, \revc{\paramAfilterrate}}$
      \li $\patLCA \gets \Call{LCA}{\maptSample, A_{cat}}$ \label{alg-line:mapt-lca} \Comment{from \cite{DBLP:journals/pvldb/GebalyAGKS14}}
      \li $\maptTODO \gets \Call{pickTopK}{\patLCA,\maptKcat,\maptAPT}$ \label{alg-line:cat-top-k}
      \li $\maptDONE \gets \emptyset$
      \li \While $\maptTODO \neq \emptyset$ \label{alg-line:mapt-refine}
         \Do
         \li $\maptPat \gets \Call{pop}{todo}$
         \li $\maptDONE \gets \maptDONE \cup \{ \maptPat \}$
         \li \For $\tup_{cur} \in \{ \tup_1, \tup_2 \}$ \Do
             \li \If $\Call{recall}{\maptPat,\tup_{cur}} > \paramRecallThresh$ \label{alg-line:mapt-filter-recall}\Then
                 \li \If $\Call{F1}{\maptPat,\tup_{cur}} > \Call{F1}{\textsc{peek}(\explset)}$ \Then
                     \li $\explset \gets \Call{deleteMin}{\explset}$
                     \li $\explset \gets \Call{insert}{\explset, (\maptPat, \tup_{cur})}$
                     \End
                 \li \For $A \in \maptAnum$ \Do
                     \li \If $\maptPat.A = \placeh$ \Then
                         \li \For $op \in \{=, \leq\}, c \in \Call{getFragments}{\domOf{APT}{A}}$ \Do
                              \li $\maptPatnew \gets \maptPat$
                              \li $\maptPatnew.A \gets \patop{op}{c}$
                              \li \If $\maptPatnew \not\in done$ \Then
                                  \li $\maptTODO \gets \maptTODO \cup \{ \maptPatnew \}$
                              \End
                         \End
                      \End
                  \End
             \End
          \End
      \End
    \li \Return $\explset$
    \end{codebox}
    \begin{codebox}
      \Procname{$\proc{\maptFilterAttrs}(\maptAPT, \paramAfilterrate)$}
      \li $A \gets \schemaOf{\maptAPT}$
      \li $\maptAfilter \gets \Call{filterBasedOnRelevance}{\maptAPT, \paramAfilterrate}$ \label{alg-line:mapt-filter-attrs-relevance}
      \li $\maptCluster \gets \Call{clusterAttributes}{\maptAfilter, \maptAPT}$ \label{alg-line:mapt-filter-attrs-cluster}
      \li $\maptArepresent \gets \Call{pickClusterRepresentatives}{\maptCluster, \maptAPT}$ \label{alg-line:mapt-filter-attrs-pick-representatives}
      \li $\maptAnum \gets \{ A \mid A \in \maptArepresent \land A \mathtext{is numeric} \}$
      \li $\maptAcat \gets \{ A \mid A \in \maptArepresent \land A \mathtext{is categorical} \}$
      \li \Return $(\maptAnum, \maptAcat, \maptCluster)$
    \end{codebox}
    }
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We give an overview of
%present
our algorithm %(\Cref{alg:basic-pattern-mine})
for mining patterns from an augmented provenance table
(\abbrAPT) generated based on a given join graph $\jgraph$. Recall that we are dealing with patterns that may contain
equality comparisons (for categorical attributes) and/or inequality comparisons (for numeric attributes). %Inequality comparisons are only considered for numerical attributes.
We mine patterns in multiple
phases. (i) In the first {\em preprocessing step},
we {\em cluster attributes} that
are highly correlated to reduce redundancy in the patterns.
The output of this %preprocessing
step are %the generated
clusters each with one selected
representative. %(\Cref{alg:basic-pattern-mine}, function \proc{\maptFilterAttrs}),
% we use random forests to determine the
% relevance of each attribute on predicting tuples to belong to the provenance of
% one of the two data points from the user's question.
% The purpose of this step is to remove attributes that
% are unlikely to yield patterns of high quality. Then we cluster attributes that
% are highly correlated to reduce redundancy in the generated patterns.
(ii) In the second preprocessing step, we use random forests to remove clusters that have low relevance on predicting
membership of input tuples in the provenance of
only one of the two output tuples from the user question. Such attributes are unlikely to yield patterns of high quality.
(iii) Next %of pattern mining,
%(line~\ref{alg-line:mapt-lca} and following)
we only consider categorical attributes and mine pattern candidates using a
variation of the \emph{LCA (Least Common Ancestor)} method from~\cite{DBLP:journals/pvldb/GebalyAGKS14} that can only handle categorical attributes. (iv) From the set of patterns returned by the LCA method, we then select the  top-$\maptKcat$ patterns with the highest recall and frequency for the next step. % (line~\ref{alg-line:cat-top-k}).
%\red{CHECK} %\red{Add the full form of LCA and a line on the summary of this method.} (iii) From the set of patterns generated in this fashion we then select a subset of further consideration \red{HOW??}.
(v) These patterns are then \emph{refined} (see below)
%(line~\ref{alg-line:mapt-refine} and following)
by adding conditions on
numerical attributes that can improve precision at the potential cost of
reducing recall. 
% (vi) The refined patterns are filtered to remove patterns with
% recall below a threshold $\paramRecallThresh$.
%(line~\ref{alg-line:mapt-filter-recall})
(vi) Finally, the top-k patterns based on score according
to~\Cref{def:metrics} are returned.
%Finally, the top-k patterns according to this ranking are returned. % The full algorithm is shown
% in~\Cref{alg:basic-pattern-mine}.

%Before describing the individual steps of our pattern mining algorithm, we first need to introduce additional notation used in this section.
%Given a pattern $\pat$,
A pattern $\pat'$ is a {\bf refinement} of a pattern $\pat$ if $\pat'$ can
be derived from $\pat$ by replacing one or more %placeholders (
$\placeh$ with
comparisons, e.g., pattern $\pat_2 = (\peq{X}, \pleq{Y})$ is a
refinement of $\pat_1 = (\peq{X}, \placeh)$.
%\BG{Adapt if we do not get to  that.}
We use following observation that follows from \Cref{def:metrics} (a), (b), (d), and (e) to prune patterns if their recall
is below a threshold.
%%%%%%%%%%%%%%%%%%%%
  \begin{proposition}
 % Using Definition~\ref{def:metrics}, g
 Given a tuple $t \in Q(D)$ and a join graph $\jgraph$, $\Rec(\sexpl_2, \jgraph,  \tup)
\leq \Rec(\sexpl_1, \jgraph,  \tup)$, where $\sexpl_1 = (\jgraph, \pat_1)$, $\sexpl_2 = (\jgraph, \pat_2)$, and $\pat_2$ is a refinement of $\pat_1$.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%
%   \begin{proof}
%   Following Definition~\ref{def:metrics} (a), if a $\tup' \in \pt{\query, \db, \tup}$ is covered by $\sexpl_2$, then it is also covered by $\sexpl_1$. Hence, by (b) and (d),  $\ITP(\sexpl_1, \jgraph, \tup) \geq \ITP(\sexpl_2, \jgraph, \tup)$ and $\IFN(\sexpl_1, \jgraph, \tup) \leq \IFN(\sexpl_2, \jgraph, \tup)$. Therefore, using (e), $\Rec(\sexpl_2, \jgraph,  \tup)
% \leq \Rec(\sexpl_1, \jgraph,  \tup)$.
%   \end{proof}
    \cut{
    \begin{proof}
      Directly following Definition~\ref{def:metrics} (a), (b), (d), and (e).
    \end{proof}
    }
 % Since if a tuple  that the recall of a refined pattern has to be less than or equal to the recall of the pattern it is derived from \red{NEED A PROPOSITION?}.
%We exploit the above fact to exclude patterns and their refinements early %on in the process if their recall is below a threshold.
Next we discuss the above six steps in detail.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Filtering and Clustering Attributes}
%\subsubsection{Filtering and Clustering Attributes}
%\label{sec:filt-clust-attr}

\cut{
Before mining patterns, we analyze the attributes of an \abbrAPT to (1) determine the attributes that are unlikely to contribute to top-k patterns because they are not helpful in distinguishing between the two outputs of interest in the user question, and (2) to identify clusters of attributes with strong mutual correlations, because such attributes can lead to redundancy in explanations as discussed below.
%The pseudo code for method $\proc{\maptFilterAttrs}$ implementing this step is shown in~\Cref{alg:basic-pattern-mine}. %\red{need to mention procedure names from the pseudocode to the corresponding method in text}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Clustering Attributes based on Correlations}\label{sec:clust-attr}
Redundancy in patterns can be caused by attributes that are highly correlated. As an extreme example, consider an \abbrAPT containing both the birth date and age of a person. For any pattern containing a predicate on birth date there will be an (almost) equivalent pattern using age instead, and also a pattern using  both age and birth date. To reduce the prevalence of such redundant patterns, we cluster attributes based on their mutual correlation
%(line~\ref{alg-line:mapt-filter-attrs-cluster})
and pick a single representative for each cluster.
%(line~\ref{alg-line:mapt-filter-attrs-pick-representatives}).
We use VARCLUS~\cite{sarle1990sas}, a clustering algorithm closely related to principal component analysis and other dimensionality reduction techniques~\cite{roweis2000nonlinear}. However, any technique that can cluster correlated attributes would be applicable.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Filtering Attributes based on Relevance}
\label{sec:filt-attr}
Random forests have been successfully used in machine learning applications  to determine the relevance of a feature (attribute) to the outcome of a classification task.
We train a random forest classifier
%(line~\ref{alg-line:mapt-filter-attrs-relevance})
that predicts whether a row belongs to the augmented provenance of only one of the two outputs from the user's question~\cite{breiman2001random}. %\BG{Cite some work that discusses using random forests to rank features}
% We then rank attributes based on the relevance and find the fraction $\paramAfilterrate$ of attributes with the highest relevance ($\paramAfilterrate$ is a threshold used by the system).
We then find the fraction $\paramAfilterrate$ of attributes with the highest relevance ($\paramAfilterrate$ is a threshold used by \oursystem, a summary of all parameter discussed in this section is shown in  \Cref{tab:exper_para}).
The rationale for this step is to prune patterns involving attributes that are irrelevant for distinguishing the  tuples $t_1, t_2$ from the user question.  % and thus reduce the search space for patterns, and additionally exclude attributes that are mostly the same in the APT of the two outputs.
%Such attributes can be added to any pattern with minimal effect on the recall and precision of patterns, since they essentially do not affect the matches for the patterns. This could mislead users into thinking that the value of this attribute is a distinguishing factor for the tuples in the user question when in fact the value of this attribute has very limited or no effect.
Such attributes can be added to any pattern with minimal effect on the recall and precision of patterns,
but could mislead users into thinking that the value of this attribute is a distinguishing factor for $t_1, t_2$.
%the tuples in the user question.
%when they essentially have very limited or no effect on the matches for the patterns.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{%Generating
% Patterns over Categorical Attributes}
\subsubsection{Patterns over Categorical Attributes}
\label{sec:gener-patt-over}

We then generate a sample of size $\paramPatsamplerate$ (an input parameter) from %\abbrAPT
$\jtr(Q, \db, \jgraph)$
%(line~\ref{alg-line:mapt-sample})
and
a set of candidate patterns over only categorical attributes using the LCA method
from~\cite{DBLP:journals/pvldb/GebalyAGKS14}. We ignore all
numerical attributes at this stage by using $\placeh$.
%(line~\ref{alg-line:mapt-lca}).
The LCA method generates pattern
candidates from a sample by computing the cross product of the sample with
itself.
%\red{not clear -- need a few more lines on LCA method}.
A candidate pattern is generated for each pair $(t,t')$ of tuples from
the sample by replacing values of attributes $A$ where $t.A \neq t'.A$ with a
placeholder $\placeh$ and by keeping constants that $t$ and $t'$ agree upon
($t.A = t'.A$). Note that in our case each element of a pattern is a
predicate, therefore, using a constant as done in the LCA method corresponds to using
an equality predicate (i.e., $A = c$ for $t.A = t'.A = c$). By keeping constants
that frequently co-occur, the LCA method
%that only works for categorical attributes (equality comparisons)
generates patterns that reflect common
combinations of constants in the data.
%Note that we ignore numeric attributes at this step, i.e., we use $\placeh$ for all numeric attributes.
%We use $\placeh$ for all numeric attributes at this step.
% The rationale of focusing on categorical attributes first is that we can (i) use the
% established heuristic of the LCA method to generate pattern candidates from categorical attributes, and (ii) we can
% significantly reduce the search space by pruning all refinements of patterns
% that fail to have a sufficiently high recall.
Focusing on categorical attributes first enables us to (i) use the
established heuristic of the LCA method to generate categorical-only pattern candidates,
and (ii) to significantly reduce the search space by pruning all refinements of patterns
without a sufficiently high recall. %\ZM{add LCA frequency pruning?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Filtering Categorical Pattern Candidates}
\subsubsection{Filtering Categorical Pattern Candidates}
\label{sec:filt-categ-patt}

Next, we calculate the recall for each pattern %by filtering the APT
finding the matches for the pattern in the \abbrAPT. As an optimization, we calculate the
recall over a sample of the data (with sample size
% $\paramQualitysamplerate$). %Note that we use
$\paramFscoresamplerate$).
Note that $\paramFscoresamplerate$ can be different from the sample size $\paramPatsamplerate$ in the previous step
%    This may require using a separate sample size
%($\maptKcat$)
%($\paramPatsamplerate$)
since we found that a small sample is sufficient for generating a meaningful set of
patterns, but may not be sufficient for estimating recall accurately enough.
%with high enough accuracy.
%\BG{In the implementation we use a sample rate plus some lower and upper bound on the sample size. Describe this here or keep it simple?}
Irrespective of whether the recall is calculated exactly  or estimated, we then filter
out patterns whose recall is below a threshold $\paramRecallThresh$,
%and pick the top patterns based on their recall.
and pick the top-$\maptKcat$ patterns based on their frequency and recall, which we denote by $\patLCA$.
%\BG{We use frequency of the pattern in the LCA result in the implementation, what to do about that?}
%In the following w
%We use $\patLCA$ to denote the set of patterns that are returned by this step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Refinement and Numeric Attributes}
\subsubsection{Refinement and Numeric Attributes}
\label{sec:pattern-refinement}
We then generate refinements of patterns from $\patLCA$ by filling placeholders $\placeh$ on numerical attributes with predicates. Even though such refinements can at best have the same recall as the original pattern, their precision may be higher resulting in greater \abbrFs. Recall that for numerical attributes we allow for both equality as well as inequality predicates, for which there is a large number of possible constants to choose from due to the large domain of numerical attributes. To reduce the size of the search space, we split the domain of each numerical attribute into a fixed number of
% $\paramNumRefineFrags$
%equally-sized
fragments (e.g., quartiles) and only use boundaries of these fragments when generating refinements.
%For example, we would use $25\%, 50\%, 75\%$ value of an attribute's domain.
% for $\paramNumRefineFrags = 3$ we would use the minimum, median, and maximum value of an attribute's domain.
We systematically enumerate all refinements of a pattern by extending it by one predicate at a time.
% For each such refinement we calculate its recall as described above and stop further refining when the recall is below $\paramRecallThresh$.
%Patterns whose recall is below $\paramRecallThresh$ are not further refined.
We use $\patset_{refined}$ to denote the union of $\patLCA$ with the set of patterns generated in this step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Computing Top-k Patterns}
\subsubsection{Computing Top-k Patterns}
\label{sec:computing-top-k}


\newcommand{\wscore}{\textsc{wscore}}
\newcommand{\dscore}{\mathcal{D}}
\newcommand{\patres}{\mathcal{R}}
\newcommand{\dmatchs}{\textsc{matchscore}}

\iftechreport{
Finally, we calculate the \abbrFs for each pattern in $\patset_{refined}$ and return $k$ patterns as follows.
\revm{To improve the diversity of the returned patterns we rank them based on a score that combines \abbrFs (\Cref{def:metrics}) with a diversity score $\dscore(\pat,\pat')$ that measures how similar two patterns are. The first pattern to be returned is always the one with the highest \abbrF. Then we determine the $i+1^{th}$ pattern based on this score. Note that the diversity score $\mathcal{D}(\pat)$ for a pattern $\pat$ depends on the set $\mathcal{R}$ of patterns we have selected to far, because it measures how close the pattern $\pat$ is to the most similar pattern in $\mathcal{R}$. We calculate this as a score $\dscore(\pat,\pat')$ that ranges between -2 and 1 (larger scores means that the two patterns are more dissimilar).
The formula for calculating the score is shown below.  For each attribute $A$ of pattern $\pat$ we add 1 if the attribute does not appear in $\pat'$, we add a penalty (-0.3) if the attribute appears in both patterns (but with different constants), and a larger penalty (-2) if it appears in both patterns with the same constant. We repeatedly add the pattern with the highest score to $\mathcal{R}$ until we have $k$ patterns to return.} % include for each attribute $A$ of the pattern
% with the highest scores according to .
 % We use a min-heap to keep track of top-$k$ patterns, and replace the lowest of current top-$k$ if we encounter a higher \abbrF value.

{\footnotesize
\revm{
  \[ \wscore(\pat) = \fscore(\sexpl, \jgraph,  \tup_1, \tup_2) + \min_{\pat' \in \patres} \dscore(\pat,\pat') \]
  \[ \dscore(\pat,\pat') = \frac{\sum_{A: \pat.A \neq \placeh} \dmatchs(\pat,\pat',A) }{\card{\pat}}\]
  \[
    \dmatchs(\pat,\pat',A) =
    \begin{cases}
      1    & \pat'.A = \placeh        \\
      -0.3 & \pat.A[0] \neq \pat.A[0] \\
      -2   & \pat.A[0] = \pat.A[0] \\
    \end{cases}
  \]
}
}
}

\ifnottechreport{
\revm{Finally, we calculate the \abbrFs for each pattern in $\patset_{refined}$ and return $k$ patterns by taking into account both \abbrFs and a measure for diversity
%to avoid similar patterns with the same values for many attributes, and
to give the user different types of interesting explanations (details in the full version \cite{chenjie2021}).
%We denote the result of this step as $\pattopk$.
%
%\todoC{Describe our new diversity approach}
We iteratively build the final pattern set of size $k$ starting with the pattern with the highest \abbrF. When deciding what pattern to add next to the result, we penalize patterns that share attributes and values with a pattern that is already in the result.
}

\cut{
\revm{To improve the diversity of the returned patterns we rank them based on a score that combines \abbrFs (\Cref{def:metrics}) with a diversity score $\dscore(\pat,\pat')$ that measures how similar two patterns are. The first pattern to be returned is always the one with the highest \abbrF. Then we determine the $i+1^{th}$ pattern based on this score. Note that the diversity score $\mathcal{D}(\pat)$ for a pattern $\pat$ depends on the set $\mathcal{R}$ of patterns we have selected to far, because it measures how close the pattern $\pat$ is to the most similar pattern in $\mathcal{R}$. For each attribute $A$ of pattern $\pat$ we add positive value as ``reward" if the attribute does not appear in $\pat'$ and we add negative value as ``penalty" if the attribute appears in both patterns. Specifically, we add a larger penalty if the attribute and its constant are the same between $\pat$ and $\pat'$ and a smaller penalty if $\pat$ and $\pat'$ share same attribute but with different constants. We repeatedly add the pattern with the highest score to $\mathcal{R}$ until we have $k$ patterns to return.}
}
}

\vspace{-2mm}

% \section{Join Graph Enumeration}\label{sec:join-graph-enumeration}
\subsection{Join Graph Enumeration}\label{sec:join-graph-enumeration}

  \newcommand{\jgZero}{\jgraph_0}
  \newcommand{\algjgJSize}{JSize}
  \newcommand{\algjgIsValid}{isValid}
  \newcommand{\algjgAddEdge}{AddEdge}
  \newcommand{\algjgGenNewJG}{ExtendJG}
  \newcommand{\algjgExpls}{\mathcal{E}}
  \newcommand{\algjgPK}{getPK}
  \newcommand{\algjgnone}{n_1}
  \newcommand{\algjgntwo}{n_2}
  \newcommand{\algjgRels}{rels}
  \newcommand{\algjgStart}{start}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iftechreport{
\begin{algorithm}
  \caption{Join Graph Enumeration}\label{alg:join-graph-enumeration}
{\small
  \begin{codebox}
    \Procname{\proc{\JGGen}$(\jgZero, \asgraph, \query,k, k_{cat})$}
    \li $\algjgExpls \gets \emptyset$ \Comment{maps join graphs to explanations}
	\li $\jgraphs{} \gets \{\jgZero\}$ \Comment{generated join graphs}
	\li $\jgraphs{prev} \gets \{\jgZero\}$ \Comment{join graphs from the previous iteration}
	\li \While $\algjgJSize \in \{ 1, \ldots, \paramJoinGraphSize \}$ \label{alg-line:jge-main-loop}
	\li \Do $\jgraphs{new} \gets \emptyset$ \Comment{join graphs generated in this iteration}
	\li \For $\jgraph \in \jgraphs{prev}$ \Do
    \li $\jgraphs{new} \gets \jgraphs{new} \cup \proc{\algjgGenNewJG}(\jgraph,\asgraph, \query$)  \label{alg-line:jge-extend-jg}
    \End
        \li \For $\jgraph \in \jgraphs{new}$ \Do
    \li \If $\Call{\algjgIsValid}{\jgraph}$ \Then \label{alg-line:jge-test-valid}
    \li $\algjgExpls[\jgraph] \gets \Call{\algMineAPT}{\db, \jgraph, \query, t_1, t_2, k, k_{cat}}$
    \End
    \End
    \li $\jgraphs{} \gets \jgraphs{} \cup \jgraphs{new}$
    \li $\jgraphs{prev} = \jgraphs{new}$
    \End
    \li \Return $\algjgExpls$
      \end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      	\begin{codebox}
	\Procname{\proc{\algjgGenNewJG}($\asgraph, \jgraph, \query$)}
	\li $\jgraphs{new} \gets \emptyset$
	\li \For $v \in \jgraphnodes$ \Do
	\li \If $\tlabelv(v) = \ptlabel$ \Then
    \li $\algjgRels \gets \relsinQ$
    \li \Else
    \li $\algjgRels \gets \tlabelv(v)$
    \End
	\li  \For  $r \in \algjgRels, n \in \snodes{}$ \Do
       \li $e \gets (r,n)$
        	\li \If $e \in \sedges{}$ \Then \label{alg-line:extjg-iterate-edges}
        	\li \For  $c \in \sglabel(e)$ \Do
                \li $\jgraphs{new} \gets \jgraphs{new} \cup \Call{\algjgAddEdge}{\jgraph, v, n, c}$
                \End
                \End
                \End
    \End
    \li \Return $\jgraphs{new}$
  \end{codebox}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   	\begin{codebox}
   	\Procname{\proc{\algjgAddEdge}($\jgraph, v, end, cond$)}
   	\li $\jgraphs{added} \gets \emptyset$
    \li $\jgraph_{curr} \gets \jgraph$ \Comment{Add $end$ as new node}
    \li $v_{new} \gets \Call{newNode}{}, e \gets (v,v_{new})$
    \li $\jgraph_{curr}.\jgraphnodes \gets \jgraph_{curr}.\jgraphnodes \cup \{v_{new}\}$
    \li $\jgraph_{curr}.\tlabelv(v_{new}) \gets end$
    \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{e\}$
    \li $\jgraph_{curr}.\tlabele(e) \gets cond$
    \li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
    %%%%%%%%%%
   	\li \For $v' \in \jgraph.\jgraphnodes: \tlabelv(v') = end$ \Comment{Add edge connecting existing nodes} \Do
           	\li \If $\neg \exists e \in \jgraph.\jgraphedges: e = (v,v') \land \jgraph.\tlabele(e) = cond$ \Then
           	\li $\jgraph_{curr} \gets \jgraph$
            \li $e \gets (v,v')$
            \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{e\}$
            \li $\jgraph_{curr}.\tlabele(e) \gets cond$
           	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
        \End
             \End
    \li \Return $\jgraphs{added}$
   	\end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{codebox}
        \Procname{\proc{\algjgIsValid}$(\jgraph)$}
        \li \For $v \in \jgraphnodes$ \Do
        \li \For $A \in \Call{\algjgPK}{\tlabelv}$ \Do
        \li \If $\neg \exists e \in \jgraphedges: A \in \attrs(\tlabele(e))$ \Then
        \li \Return $\bfalse$
        \End
        \End
        \End
        \li \If $\Call{estimateCost}{\jgraph} > \paramMaxQcost$ \Then
        \li \Return $\bfalse$
        \End
        \li \Return $\btrue$
      \end{codebox}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
}
\end{algorithm}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%we present our algorithm for enumerating join graphs ($\algogbasic$). The
In this section,
we describe an algorithm
\iftechreport{present in  \Cref{alg:join-graph-enumeration}}
that enumerates join graphs of increasing size iteratively. %\revm{(details and pseudocode in full version)}.
% In iteration $i$, we enumerate all join
% graphs with $i$ edges by adding a single edge conforming to the schema graph to
% one of the join graphs of size $i-1$
% %produced in the previous iteration.
% from iteration $i-1$.
The
maximum size of join graphs considered by the algorithm is determined by
a parameter \paramJoinGraphSize. We employ several heuristic tests to determine
whether a join graph generated by the algorithm should be considered for pattern
mining.
% The rationale for not considering all join graphs for pattern mining is
% that pattern mining can be significantly more expensive than just generating a
% join graph, so  %Thus, we have an incentive to
% we skip pattern mining for join graphs
% that are either unlikely to yield patterns of high quality or for which
% generating the \abbrAPT and patterns are likely to be expensive.
The rationale for not considering all join graphs for pattern mining is
that for some join graphs, pattern mining may not yield  patterns of good quality, or it may be much more computationally expensive than generating the join graph. Hence
we skip pattern mining for join graphs that are unlikely to be worth the cost.
For join
graphs that pass these tests we materialize the corresponding \abbrAPT and
apply the pattern mining algorithm from \Cref{sec:algo_pattern} to compute the
top-k patterns for the \abbrAPT.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Generating Join Graphs}
\label{sec:gener-join-graphs}

\mypar{Generating join graphs} We enumerate join graphs in iteration $i$ by extending every join graph produced in iteration $i-1$ with all possible edges. For each join graph $\jgraph$ produced in iteration $i-1$, we consider two types of extensions: (i) we add an additional edge between two existing nodes of the graph and (ii) we add a new node and connect it via a new edge to an existing node.
\iftechreport{
The main entry point is function \textsc{\JGGen} from \Cref{alg:join-graph-enumeration}. We first initialize the result to contain $\jgZero$, the join graph consisting of a single node labeled ($\ptlabel$).
Within each iteration of the main loop (line~\ref{alg-line:jge-main-loop}), each join graph $\jgraph$ from the set of join graphs generated in the previous iteration ($\jgraphs{prev}$) is passed to function \proc{\algjgGenNewJG} which computes the set of all possible extensions of $\jgraph$ (line~\ref{alg-line:jge-extend-jg}). For any such join graph produced in this step, we then check whether it should be considered for patterning mining using function described below (line~\ref{alg-line:jge-test-valid}). For any join graph passing this check we call \proc{\algMineAPT} to generate the top-k patterns and store them in $\algjgExpls$.

% passing it along with the schema graph $\asgraph=\sgraph$ to \proc{\algjgGenNewJG}. \proc{\algjgGenNewJG} will add one more edge to the passed join graph (denoted as $\jgraph$) exhaustively by traversing each node in the $\jgraph$.

Function \proc{\algjgGenNewJG} enumerates all possible extension of a join graph with one additional edge. For that we consider all existing nodes $v$ in the join graph as possible extension points. We then enumerate all edges from the schema graph $\sgraph$ that are adjacent to nodes $r$ for relations that are represented by $v$. For that we have to distinguish two cases.  If $v$ is labeled $\ptlabel$, then $r$ can be any relation accessed by the query. Otherwise, there is a single node $r$ that is determined based on $v$'s label (the relation represented by $v$). For each edge $e$ adjacent to a node $r$ (line~\ref{alg-line:extjg-iterate-edges}), we then iterate over all conditions $c$ from the label of $e$ and then use function \proc{\algjgAddEdge} to enumerate all join graphs generated from $\jgraph$ by connecting $v$ with an edge labeled with $c$ to another node (either already in the join graph or new node added to the graph).

Function \proc{\algjgAddEdge} first generates a join graph by adding a new node $v_{new}$ labeled $end$ (the relation that is the end point of the edge in the schema graph) and connects it to $v$. Afterwards, for each node in the join graph $\jgraph$ labeled $end$ that is not connected to $v$ though an edge labeled $cond$ already, we generate a new join graph by adding such an edge.
}

% we consider two scenarios, one is if the node we are processing is $\ptlabel$ (line 3-10), then we will traverse $\relsinQ$ one by one. The other one is that the node is just one relation (line 11-17). Once \proc{\algjgGenNewJG} has found an valid edge to add (need to have 2 nodes $r,n$ and a condition on the edge $c$), it pass those arguments along with the $\jgraph$ being processed to \proc{\algjgAddEdge}. \proc{\algjgAddEdge} then try to first find the first node of the edge ($\tlabelv(v)==rel_1$) from $\jgraph$. Then \proc{\algjgAddEdge} traverse through $\jgraph$ see if there exists an node $\tlabelv(v')==rel_2$ and at the same time, $(v,v')$ does not exist in the edges of the $\jgraph$. If it is the case, \proc{\algjgAddEdge} will add this edge with the assignment of condition $cond$. Note in line 10-line 15 in \proc{\algjgAddEdge}, it will always add a new node $v''$ and new edge $(v,v'')$ to $\jgraph$.



% The \JGGen first starts by initializing the generated join graphs $\jgraphs{}$ as only having one join graph which only has one node contains $\ptlabel$. $\jgraphs{prev}$ denotes the generated join graph set from the previous iteration, initialized also only contains one same join graph as in $\jgraphs{}$. Then the algorithm iterates until the maximum number of operations allowed N is reached.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Checking Join Graph Connectivity and Skipping Expensive \abbrAPT Computations} \label{sec:checking-join-graph}

\mypar{Checking join graph connectivity and skipping expensive \abbrAPT computations}
We filter out join graphs based on \emph{lack of connectivity} and on \emph{high estimated costs}.
\iftechreport{
We use the function \proc{\algjgIsValid} shown in \Cref{alg:join-graph-enumeration} to filter out join graphs based on lack of connectivity (described in the following) or based on high estimated computation costs.
}Note that schema graphs may contain tables with multiple primary key attributes incident to edges which join on part of the key. This is typical in
``mapping'' tables that represent relationships. For instance, consider the
{\tt PlayerGameScoring} table from our running example that stores the number
of points a player scored per game. Assume that there exists another
table {\tt Player} that is not part of the running example.  The primary key of {\tt PlayerGameScoring} consists of a foreign key to the {\tt Game} table and a foreign key to the {\tt Player} for
which we are recording stats. 
% For this example also assume that the
% schema graph permits that {\tt PlayerGameScoring} to be joined with the {\tt Player} table.
Consider a query that joins the {\tt Game} table with {\tt LineupPerGameStats},
{\tt LineupPlayer} and selects games played by team GSW. A valid
join graph for this query would be to join the node $\ptlabel$ with
{\tt PlayerGameScoring} on game's primary key.

Note that while the result of this
query contains rows that pair a player of GSW with lineups they played in during a
particular game, the \abbrAPT would pair each row with any player that played in
that game irrespective of their team. Join graphs like this can lead to
redundancy and large \abbrAPT tables. One reason for this redundancy is that not
all primary key attributes of the {\tt PlayerGameScoring} table are joined with
another table. To prevent such join graphs with redundancy,
%function \proc{\algjgIsValid}
our algorithm checks that
for every node in the join graph, the primary key attributes of
%the relation corresponding to
that node are joined with at least one other node from the join
graph. For instance, in the example above the join graph could be modified to
pass this check by also joining the {\tt PlayerGameScoring} table with the {\tt Player}
table.

Even though we only consider fully connected join graphs, some generated
join graphs will result in \revc{\abbrAPT}s of significant size, which are expensive to
materialize and mine patterns from.
%Recall that we use queries to materialize join graphs.  We use the DBMS to estimate the cost of this query upfront.
We use the DBMS to estimate the cost of the materialization query upfront.
We skip pattern mining for join graphs where the estimated cost of this query is
above a threshold $\paramMaxQcost$. While we may lose explanations by skipping
join graphs, experimental results demonstrate that this check is necessary for
achieving reasonable performance. \reva{Furthermore,
%a limitation of join graph size is not unreasonable, %because a user has to comprehend both the pattern as well as the join graph to understand an explanation. Thus,
smaller join graphs result in less complex explanations. % likely not to overload the user with too complex explanations.
}\\[-2mm]
% \ZM{any discussions on $\paramMaxQcost$ ?}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Skipping Expensive \abbrAPT Computations}
% \label{sec:skipp-expens-abbr}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Ranking Results} \label{sec:ranking-results}
\mypar{\revc{Ranking results}} \revc{After enumerating join graphs and computing top-$k$ patterns for each join graph, we rank the union of all pattern sets on their \abbrF. %We decided to rank patterns % rather than filter patterns
Ranking all these patterns (instead of filtering out some patterns)
reduces the load on the user by increasing the likelihood that good patterns are shown early on without having the risk of %completely filtering out
not showing patterns that have lower scores.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Computing \abbrAPTs}
% \label{sec:computing-abbrapts}



% \BG{OLD:}
% It takes 4 parameters as input. the schema graph $\asgraph$, a join graph $\jgraph_0$ which only has one node labeled as $\ptlabel$, the maximum number of operations allowed N when constructing a join graph from $\ptlabel$, and the set of relations accessed by query $\relsinQ$. Note here we define an ``operation'' as either adding an edge along with a new node if this node from the edge does not exist in the current join graph, or adding an edge without adding a new node.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{\algogbasic}
% {\small
% 	\begin{codebox}
% 	\Procname{\JGGen($\jgraph_0$, $\asgraph$, $\relsinQ$,N)}
% 	\li $\jgraphs{}$ $\gets \{\jgraph_0\}$ \Comment{generated join graphs}
% 	\li $\jgraphs{prev} \gets$ \{$\jgraph_0$\} \Comment{Initialize previous step set}
% 	\li JSize $\gets 1$
% 	\li \While JSize $\leq N$
% 	\li \Do $\jgraphs{new} \gets \emptyset$ \Comment{new join graphs we get in this iteration}
% 	\li \For $\jgraph$ in $\jgraphs{prev}$
%         \li \Do  $\jgraphs{new} \gets \jgraphs{new} \cup$ \proc{\algjgGenNewJG}($\jgraph,\asgraph, \relsinQ$)
%             \End
%             \li $\jgraphs{} \gets \jgraphs{} \cup \jgraphs{new}$
%             \li $\jgraphs{prev} = \jgraphs{new}$
%             \li JSize  $\gets$ JSize + 1
%         \End
%         \li \Return $\jgraphs{}$
%       \end{codebox}
%       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	\begin{codebox}
% 	\Procname{\proc{\algjgGenNewJG}($\asgraph, \jgraph, \relsinQ$)}
% 	\li $\jgraphs{new} \gets \emptyset$
% 	\li \For $v \in \jgraph.\jgraphnodes$
% 	\li \Do \If $\tlabelv(v) == \ptlabel$
% 	\li \Then \For  $r \in \relsinQ$
%         \li \Do \For  $n \in \asgraph.\snodes{}$
%         	\li \Do \If (($r, n) \in \asgraph.\sedges{}$)
%         	\li \Then \For  $c \in \sglabel((r, n))$
%             \li \Do $\tlabele((r,n))=c$
%             \li $\jgraphs{added} \gets $\proc{\algjgAddEdge}($\jgraph, \ptlabel, n, c$)
%             \li $\jgraphs{new} \gets \jgraphs{new} \cup \jgraphs{added} $
%                 \End
%             \End
%         \End
%     \End
%     \li \Else $r \gets \tlabelv(v)$
%     \li \For $n \in \asgraph.\snodes{}$
%     \li \Do \If (($r, n) \in \asgraph.\sedges{}$)
%     \li \Then \For  $c \in \sglabel((r, n))$
%     \li \Do $\tlabele((r,n))=c$
%     \li $\jgraphs{added} \gets $\proc{\algjgAddEdge}($\jgraph, r, n, c$)
%     \li $\jgraphs{new} \gets \jgraphs{new} \cup \jgraphs{added} $
%                 \End
%             \End
%         \End
%     \End
%     \End
%     \li \Return $\jgraphs{new}$
%   \end{codebox}
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    	\begin{codebox}
%    	\Procname{\proc{\algjgAddEdge}($\jgraph, rel_1, rel_2, cond$)}
%    	\li $\jgraphs{added} \gets \emptyset$
%    	\li \For $v \in \jgraph.\jgraphnodes$
%        	\li \Do \If $\tlabelv(v) == rel_1$
%            	\li \Then \For $v' \in \jgraph.\jgraphnodes$
%            	\Comment{\tiny Loop throught existing nodes see if $rel_2$ already exists in $\jgraph$}
%            	\li \Do \If $\tlabelv(v') == rel_2$ {\bf and} $(v,v') \notin \jgraph.\jgraphedges$
%            	\li \Then $\jgraph_{curr} \gets \jgraph$
%            	\li $\tlabele((v,v')) \gets cond$
%            	\li $\jgraph_{curr}.\jgraphedges \cup \{(v,v')\}$
%            	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
%     \End
%         \End
%        	\li $\jgraph_{curr} \gets \jgraph$
%         \Comment{\tiny No matter if this edge exist already, add a new edge with ($rel_1, rel_2$) here}
%         \li $v'' \gets \tlabelv^{-1}(rel_2)$
%         \li $\jgraph_{curr}.\jgraphnodes \gets \jgraph_{curr}.\jgraphnodes \cup \{v''\}$
%         \li $\tlabele((v,v')) \gets cond$
%         \li $\jgraph_{curr}.\jgraphedges \gets \jgraph_{curr}.\jgraphedges \cup \{(v, v'')\}$
%        	\li $\jgraphs{added} \gets \jgraphs{added} \cup \{\jgraph_{curr}\}$
%             \End
%                \End
%     \li \Return $\jgraphs{added}$
%    	\end{codebox}
% }
% \end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/diff_summary.tex <==
\section{Summarization for Comparison (difference)}
\begin{itemize}
    \item Are we summarizing tuples from the difference only? Do differences in the join result?
\end{itemize}

As motivated in our running example, given an aggregate query, a user may not only wonder why a particular aggregation result to be unusually low or high, but also asks why an result is lower or higher than another one, which we formally define below.

\begin{definition}[User Question with Comparison]
Given a database $D$ and an aggregate query $Q$,
a user question (UQ) $\phi = (t_1, t_2, dir)$ involves two result tuples $t_1, t_2 \in Q(D)$ and a direction $dir \in \{high,low\}$ where $t_1.\aggval >$ (or $<$, resp.) $t_2.\aggval$ if $dir = high$ (or $low$, resp.)
\end{definition}

To answer such user questions with comparison, \oursys{} would first summarize the provenance for both tuples of interest, and then combine these summarizations to provide explanations to the user question.


\begin{Definition}[Join-augmented Explanation]
Given a database $D$, a join graph $G$ for $D$, a query $Q$, and two output tuples $t_1, t_2$ of interest in the answer of $Q(D)$, a constant $K$, and the join-augmented summarizations {\bf $S_1$} = ({\bf$ \jgraph_1$}, {\bf $P_1$}) for $t_1$ and {\bf $S_2$} = ({\bf$ \jgraph_2$}, {\bf $P_2$}) for $t_2$
a join-augmented explanation $e$ is
\begin{itemize}
    \item a pattern $p_1 \in \bf P_1$ but not in $\bf P_2$, and the coverage of $p_1$ for tuples in the provenance of $t_2$;
    \item a pattern $p_1 \in \bf P_3$ but not in $\bf P_1$, and the coverage of $p_1$ for tuples in the provenance of $t_1$;
    \item a pattern $p_1 \in \bf P_1$ and a pattern $p_2 \in \bf P_2$, where $p_1 \neq p_2$ and they have the same schema.
\end{itemize}
\end{Definition}

\ZM{Need to define coverage or use some other metric here.}
\ZM{For instance, if dir=low, the first two cases captures the patterns summarizing why t1 is low but not affecting t2 or why t2 is high but not affecting t1 (by showing coverage is low); the third case captures the change in the values, e.g., the performance of Curry improves a lot from 2011-12 to 2015-16.}

==> sections/optimizations.tex <==
\section{Optimizations and Implementations}
What we need to solve/address
\begin{itemize}
    % \item Numerical ranges selection
    % \item Feasible algorithm which does not guarantee for the optimal solution but reasonable results with acceptable cost: Looking into \textit{Metaheuristics}
    \item No comprehensive set of rules to avoid duplicates and enumerate all possible join graphs. Current workaround: Firstly, we filter out join graphs that don't have each node's primary key ''slots" filled. The reason is that without fully established join for primary keys, it is almost inevitable to generate cross product or partial cross product. We later realize this rule is still not enough because there are certain scenarios that can fulfill this requirement but from multiple different nodes which doesn't guarantee to preserve the constraint posed from the original provenance table. Secondly, to further avoid cross product, we implemented a ``cost estimation" step, which would avoid materializing the join graph and generating patterns from it. currently these kinds of join graphs were chosen if its cost estimate is significantly higher than the average of the whole group of join graphs which have the same number of edges. 
    % \item Consider the effectiveness of a certain ``group" of patterns, e.g. standard deviation of replacing a certain predicate with another value of the domain
    \item Enumerate patterns and also evaluate the scores are one dominating factor that affects the total running time. How to effectively decrease the number of patterns and at the same time don't lose interesting patterns? Current solution: we have a few options:
    \begin{itemize}
        \item Regression on numerical data to get the importance rankings of the attributes
        \item Random Forest
        \item Clustering of the attributes and pick at most one attribute from each cluster (currently based on the ranking of the entropy)
    \end{itemize} 
    % \item Evaluate the complexity of a join graph before actually performing the join?
    % \item Establish a tree/graph structure among the trees generated so that we could cut off branches/connections based on calculated bounds
\end{itemize}

We optimize stuff here \cite{alomeirsummarizing}, \cite{wanderj}, \cite{wu13}, \cite{prosumrev}


==> sections/quality--old.tex <==
\subsection{Quality Measure of Explanations}
%\textbf{Quality measure of summarization patterns for a given join graph.~}
First, we discuss the quality measures for explanations when the join graph is given, and then discuss how to find top explanations across all join graphs mined by our algorithms \blue{DO}.
For both single-point questions and two-point questions, we would like the patterns to be descriptive of the provenance of the single output tuple or one of the two output tuples respectively. That is, they should cover as much provenance as possible and ideally should not match anything that is not in the provenance. For this purpose, we adapt the standard notion of \emph{\abbrF}, which is a popular measure for the accuracy of a test.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Note that a tuple $\tup'$ in the provenance table can be augmented into multiple tuples in the augmented provenance table, and thus we evaluate the coverage of a pattern on both the original provenance table and augmented provenance table instead of the original provenance table. Recall that {\upshape$\matches(\pat,\rel)$} denotes $\{ \tup \in \rel \mid  \tup \pmatch \pat \}$.

\cut{
\begin{itemize}
    \item Define TP (fractional and integral)
    \item Define FP (fractional and integral)
    \item Define FN (fractional and integral)
     \item Define Recall as TP/TP+FN (fractional and integral)
      \item Define Precision as TP/TP+FP (fractional and integral)
       \item Define \abbrF as harmonic mean of Recall and Precision (fractional and integral)
\end{itemize}
}


\begin{Definition}[Coverage]\label{def:cover}
Consider a database $\db$, an \termAggJoinQ\ $\query$, a join graph $\jgraph$, a tuple
$\tup \in Q(D)$,
%$\tup \in \pt{\query, \db}$
and an explanation pattern $\sexpl = (\jgraph, \pat)$.

(a) A tuple $\tup' \in \pt{\query, \db, \tup}$ is said to be covered by $\sexpl$ if there exists $\tup''\in \jtr(\query, \db, \jgraph, \tup, \tup')$ (ref. Definition~\ref{def:apt}) such that $\tup'' \pmatch \pat$.
%Based on the way to calculate the coverage of an explanation $\sexpl$, we define two versions of the coverage of $\sexpl$.
%The \emph{integral coverage}
The \emph{coverage} of $\sexpl$ on $\tup, \tup'$ in $\jtr(Q, \jgraph, \db)$ is defined as: $$\ICov(\sexpl, \tup, \tup') = \mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup, \tup') \big) \neq \emptyset]$$
  where $\mathbb{1}[]$ is the indicator function.
  \cut{

  The \emph{fractional coverage} of $\sexpl$ on $\tup'$ in $\jtr(Q, \jgraph, \db, \tup')$ is defined as the fraction of tuples in $\jtr(\query, \db, \jgraph, \tup')$ matched by $\pat$:
 $$\FCov(\sexpl, \tup') = \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}$$
}
\end{Definition}
%\SR{There is no mention of $t$ in the above defn.}
%\CL{Modified}


\cut{
Alternatively, the fractional coverage exploits more information in the augmented provenance as a tuple is ``partially'' covered by a pattern and the fraction is based on how many tuples can be augmented from this tuple.
}

\begin{Definition}[Coverage of a Patterns: True Positive]\label{def:true-positive}
The coverage (True Positive) of $\sexpl$ is defined as sum of its coverage on all tuples in provenance:\\
For integral version, the coverage of an explanation $\ITP(\sexpl)$ is defined as:
\begin{align*}
\ITP(\sexpl) &= \sum_{\tup' \in \pt{\query, \db, \tup}} \ICov(\sexpl, \tup')\\
&= \sum_{\tup' \in \pt{\query, \db, \tup}}
\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]
\end{align*}

\cut{
For fractional version, the coverage of an explanation $\FTP(\sexpl)$ is defined as:
\begin{align*}
\FTP(\sexpl) &= \sum_{\tup' \in \pt{\query, \db, \tup}} \FCov(\sexpl, \tup')  \\
&= \sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}\\
\end{align*}
}
\end{Definition}

The %integral
coverage means a tuple in provenance is fully covered as long as there exists a tuple in the augmented provenance covered by the pattern, is the same as normal cases of summarization rules.


\begin{Definition}[Covered Tuples not in Provenance: False Positive]\label{def:false-positive}
The False Positive of $\sexpl$ is defined as sum of its coverage on all tuples not in the provenance of $\tup'$:\\
For integral version, the covered tuples not in provenance $\IFP(\sexpl)$ is defined as:
\begin{align*}
\IFP(\sexpl) &= \sum_{\tup' \in \pt{\query, \db} \setminus \pt{\query, \db, \tup}} \ICov(\sexpl, \tup')\\
&= \sum_{\tup' \in \pt{\query, \db} \setminus \pt{\query, \db, \tup}}
\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]
\end{align*}
For fractional version, the covered tuples not in provenance $\FFP(\sexpl)$ is defined as:
\begin{align*}
\FFP(\sexpl) &= \sum_{\tup' \in \pt{\query, \db} \setminus \pt{\query, \db, \tup}} \FCov(\sexpl, \tup')  \\
&= \sum_{\tup' \in \pt{\query, \db} \setminus \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}\\
\end{align*}




\end{Definition}

\SR{Add a comment that the numerators are disjoint in TP and FP even for APT as they are augmenting PT}
\CL{adding: Note that $\tup'$ from $FP(E)$ are different from $\tup'$ from $TP(E)$ as they are from two sets that complement each other}
\begin{Definition}[Uncovered Tuples in Provenance: False Negative)]\label{def:false-negative}
The False Negative of $\sexpl$ is defined as the sum of ``uncoverage'' ($1-coverage$) of tuples in the provenance of $\tup$:\\
For integral version, the covered tuples not in provenance $\IFN(\sexpl)$ is defined as:
\begin{align*}
\IFN(\sexpl) &= \sum_{\tup' \in \pt{\query, \db, \tup}} 1-\ICov(\sexpl, \tup')\\
&= \sum_{\tup' \in \pt{\query, \db, \tup}}
\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) = \emptyset]
\end{align*}
\cut{
For fractional version, the covered tuples not in provenance $\FFN(\sexpl)$ is defined as:
\begin{align*}
\FFN(\sexpl) &= \sum_{\tup' \in \pt{\query, \db, \tup}} 1-\FCov(\sexpl, \tup')  \\
&= \sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid - \mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}\\
\end{align*}
}
\end{Definition}

\begin{Definition}[Precision, Recall, and \fscore]\label{def:fscore}
With Definition~\ref{def:true-positive}, \ref{def:false-positive}, and \ref{def:false-negative}, we define precision, recall, and \fscore\ as usual:
\begin{align*}
\Prec(\sexpl) = \frac{TP(\sexpl)}{TP(\sexpl) + FP(\sexpl)}\\
\Rec(\sexpl) = \frac{TP(\sexpl)}{TP(\sexpl) + FN(\sexpl)}\\
\fscore(\sexpl) =\frac{2}{\frac{1}{\Prec(\sexpl)} +\frac{1}{\Rec(\sexpl)}}
\end{align*}

% \FPrec(\sexpl) &= \frac{\FTP(\sexpl)}{\FTP(\sexpl) + \FFP(\sexpl)}  \\
% &= \frac{\sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}}{\sum_{\tup' \in \pt{\query, \db}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}} \\
% \IPrec(\sexpl) &= \frac{\ITP(\sexpl)}{\ITP(\sexpl) + \IFP(\sexpl)}  \\
% &=\frac{\sum_{\tup' \in \pt{\query, \db, \tup}}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}{\sum_{\tup' \in \pt{\query, \db}}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}

% \begin{align*}
% \FRec(\sexpl) &= \frac{\FTP(\sexpl)}{\FTP(\sexpl) + \FFN(\sexpl)}  \\
% &= \frac{\sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}}{\sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \jtr(Q, \db, \jgraph, \tup')\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}} \\
% &= \frac{\sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}}{\mid \pt{\query, \db, \tup} \mid} \\
% \IRec(\sexpl) &= \frac{\ITP(\sexpl)}{\ITP(\sexpl) + \IFN(\sexpl)}  \\
% &=\frac{\sum_{\tup' \in \pt{\query, \db, \tup}}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}{\mid \pt{\query, \db, \tup} \mid}
% \end{align*}
% \begin{align*}
% \Ffscore(\sexpl) &=\frac{2\FPrec(\sexpl)\FRec(\sexpl)}{\FPrec(\sexpl) + \FRec(\sexpl)} \\
% \Ifscore(\sexpl) &=\frac{2\IPrec(\sexpl)\IRec(\sexpl)}{\IPrec(\sexpl) + \IRec(\sexpl)} \\
% \end{align*}
% $$\Ffscore(\sexpl) =\frac{2}{\frac{1}{\FPrec(\sexpl)} +\frac{1}{\FRec(\sexpl)}} $$
\end{Definition}


%when there are one-to-many joins.
Here since those formulas are the same for both coverage versions, we leave out the subscripts without loss of information.

A high recall implies that the pattern $\pat$ is a good description of the tuples contributing to the output tuple $t$.

Compared to the previous single answer version, the quality of explanations for the difference between two answer tuples $\tup_1$ and $\tup_2$ is also measured using $\fscore$, with a major difference lies in the calculation of the False Positive. Firstly, we need to mark one of the two result tuple as ``True" tuple \CL{could change this later...} i.e., let's choose $\tup_1$ as ``True" tuple. The False Positive for $\tup_1$ is counted over tuples in the provenance of $\tup_2$ instead of rest tuples in the entire provenance, which intuitively means that in order to get a high \abbrF, we want to capture patterns should cover as much provenance of one result tuple(``True" tuple) ($\tup_1$) as possible but not the provenance of the other result tuple ($t_2$).

\begin{Definition}[Quality Measure for Difference]\label{def:quality-measure-diff}
Let $\dexpl = (\jgraph, \pat)$ be an explanations for $\query$,  $\db$, and two tuples $\tup_1, \tup_2$,  where the precision is defined as the percentage of tuples in $\pt{\query, \db, \tup_1}$ matching $\pat$ in the augmented provenance table over those matched tuples in $\pt{\query, \db, \tup_1} \cup \pt{\query, \db, \tup_2}$.
\begin{align*}
\FPrec(\dexpl) &= \frac{\FTP(\dexpl)}{\FTP(\dexpl) + \FFP(\dexpl)}  \\
&= \frac{\sum_{\tup' \in \pt{\query, \db, \tup_1}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}}{\sum_{\tup' \in U} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}} \\
% \IPrec(\dexpl) &= \frac{\ITP(\dexpl)}{\ITP(\dexpl) + \IFP(\dexpl)}  \\
% &=\frac{\sum_{\tup' \in \pt{\query, \db, \tup_1}}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}{\sum_{\tup' \in U}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}
\end{align*}
where $U=\pt{\query, \db, \tup_1} \cup \pt{\query, \db, \tup_2}$.

The recall and \fscore\ are defined in the same way as Definition~\ref{def:fscore}.
\begin{align*}
\FRec(\dexpl) &= \frac{\FTP(\dexpl)}{\FTP(\dexpl) + \FFN(\dexpl)}  \\
&= \frac{\sum_{\tup' \in \pt{\query, \db, \tup_1}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}}{\mid \pt{\query, \db, \tup_1} \mid} \\
% \IRec(\dexpl) &= \frac{\ITP(\dexpl)}{\ITP(\dexpl) + \IFN(\dexpl)}  \\
% &=\frac{\sum_{\tup' \in \pt{\query, \db, \tup_1}}\mathbb{1}[\matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup') \big) \neq \emptyset]}{\mid \pt{\query, \db, \tup_1} \mid}
\end{align*}
% \begin{align*}
% \Ffscore(\dexpl) &=\frac{2\FPrec(\dexpl)\FRec(\dexpl)}{\FPrec(\dexpl) + \FRec(\dexpl)} \\
% \Ifscore(\dexpl) &=\frac{2\IPrec(\dexpl)\IRec(\dexpl)}{\IPrec(\dexpl) + \IRec(\dexpl)} \\
% \end{align*}
$$\Ffscore(\dexpl) =\frac{2}{\frac{1}{\FPrec(\dexpl)} +\frac{1}{\FRec(\dexpl)}} $$

\end{Definition}

\cut{
\begin{Definition}[Coverage and Recall]\label{def:coverage-recall}
%[Quality Measure for Single Answer Given a Join Graph]\label{def:quality-metrics-single}
Consider a database $D$, an \termAggJoinQ\ $\query$, a $\tup \in \query(\db)$, a join graph $\jgraph$, and an explanation $\sexpl = (\jgraph, \pat)$.
%The quality of an explanation  for $\query$,  $\db$, and a single $\tup_1$ is measured using $F_1$ score, where
\begin{itemize}
    \item The \emph{fractional coverage} of $\sexpl$ is defined as $$\FCov(\sexpl) = \sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}$$
    \item The \emph{recall} of $\sexpl$ is defined as
%the percentage of tuples in the provenance table of $\tup_1$ matching $\pat$.
$$\Rec(\sexpl) = \frac{\FCov(\sexpl)}{|\pt{\query, \db, \tup}|} $$
% $$\Rec(\sexpl) = \frac{1}{|\pt{\query, \db, \tup}|}\sum_{\tup' \in \pt{\query, \db, \tup}} \frac{\mid \matches \big(\pat,  \jtr(Q, \db, \jgraph, \tup') \big)\mid}{\mid { \jtr(Q, \db, \jgraph,  \tup')} \mid}$$
%where $\selection_{\tup, \pt{\query, \db, \tup_1}}$ is the selection on the join graph result choosing tuples whose $\pt{\query, \db, \tup_1}$ part is equal to $\tup$.
This recall definition captures the coverage of tuples in the provenance table and the property that a tuple in the provenance table $\pt{Q, D}$ can generate multiple tuples in the augmented provenance table $\jtr(Q, \db, \jgraph,  \tup')$.
%when there are one-to-many joins.
A high recall implies that the pattern $\pat$ is a good description of the tuples contributing to the output tuple $t$.   %where different patterns may match different numbers of tuples in the join graph result.
\end{itemize}
\end{Definition}

\begin{Definition}[Precision]\label{def:precision}
\item The \emph{precision} of $\sexpl$, $\Prec(\sexpl)$, is defined as the fraction of tuples in $\jtr(\query, \db, \jgraph, \tup)$ matching $\pat$:
$$\Prec(\sexpl) = \frac{\FCov(\sexpl)}{\sum_{\tup \in \pt{\query, \db}}\mathbb{1}[ \tup \in \projection_{\att_{\ptlabel}}\matches \big(\pat, \jtr(Q, \jgraph, \db, \tup) \big) ]} $$

   The \emph{precision} of $\sexpl$, $\Prec(\sexpl)$, is defined as the fraction of tuples in $\pt{\query, \db, \tup}$ \SR{should be APT?}
    \ZM{should be PT. E.g., to summarize GSW wins, the precision of pattern (Curry pts > 30) should be \\
    $\frac{|\text{GSW win} \land  \text{Curry pts }> 30|}{|\text{GSW games with Curry pts} > 30|}$, showing how accurate the pattern is in predicting GSW win, or differentiating GSW win games and other games.}
    matching $\pat$ after being augmented using the join graph: %,  which is always 1 in this single answer case;
    $\Prec(\dexpl) = \frac{TP}{TP+FP}$ , where the numerator TP (true positive) is the total number of tuples in $\pt(Q, \db, \tup)$ matching $\pat$ after augmented $$TP = \sum_{\tup \in \pt{\query, \db, \tup_1}} \mathbb{1}[\tup \in \projection_{\att_{\ptlabel}} \matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup) \big)]$$
    and the denominator TP + FP (true positive + false positive) is the total number of tuples in the same context of $\tup_1$ matching $\pat$ after augmented. When the user query \query contains selection predicates in its {\tt WHERE}-condition $\theta$, the context of $\tup_1$ is defined as the all tuples in the provenance of other outputs of \query.
    % $$FP =  \sum_{\tup \in \pt{\query, \db, \tup_2}}\mathbb{1}[ \tup \in \projection_{\att_{\ptlabel}}\matches \big(\pat, \jtr(Q, \jgraph, \db, \tup) \big) ]$$
    $$TP+FP = \sum_{\tup \in \pt{\query, \db}}\mathbb{1}[ \tup \in \projection_{\att_{\ptlabel}}\matches \big(\pat, \jtr(Q, \jgraph, \db, \tup) \big) ]$$
    While when the user query \query\ does not have any selection predicates, the result of \query\ would enumerate all value combinations of grouping attributes, and thus we only consider $\tup_1$ itself as its context, leading to an 1 precision. A high precision implies that the pattern $\pat$ is a good discriminator for tuples contributing to the output tuple $t$ and other output tuples when the context is given.
    \end{Definition}

    \SR{don't follow this -- we talked about the impact of `WHERE' -- no where means precision 1, otherwise we need to divide by something.}
    \ZM{Correct me if wrong: if the query selects on `winner = GSW', grouping on team and season, then the context should be GSW wins in every season, and we are summarizing the difference between season 2015-16 and other seasons. }

\begin{Definition}


    As usual, the \abbrF of $\sexpl$, denoted $\fscore(\sexpl)$, is the harmoning mean of $\Rec(\sexpl)$ and $\Prec(\sexpl)$.

\end{Definition}
}
% \SR{=========UPDATED UP TO HERE =========}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cut{
\begin{Definition}[Quality Metrics for Difference]\label{def:quality-metrics-diff}
Let $\dexpl = (\jgraph, \pat)$ be an explanations for $\query$,  $\db$, and two tuples $\tup_1, \tup_2$, the quality of $\dexpl$ is also measured using $F_1$ score, where the precision is defined as the percentage of tuples in $\pt{\query, \db, \tup_1}$ matching $\pat$ in the join graph result over those matched tuples in $\pt{\query, \db, \tup_1} \cup \pt{\query, \db, \tup_2}$.

% $$ Pre(\dexpl) = \frac{\mid \matches \big(\pat, \selection_{\tup,  \pt{\query, \db, \tup_1}} \jtr(\jgraph, \pat) \big)\mid}
% {\mid \matches \big({\selection_{\tup, \pt{\query, \db, \tup_1}} \jtr(\jgraph, \pat)} \big) \mid + \mid \matches \big({\selection_{\tup, \pt{\query, \db, \tup_2}} \jtr(\jgraph, \pat)} \big) \mid}$$

%$$
% Pre(\dexpl) = \frac{\mid \matches \big(\pat, \selection_{\tup,  \att^1} \jtr(\jgraph, \pat) \big)\mid}
% {\mid \matches \big({\selection_{\tup, \att^1} \jtr(\jgraph, \pat)} \big) \mid + \mid \matches \big({\selection_{\tup, \att^2}} \jtr(\jgraph, \pat) \big) \mid}
%Pre(\dexpl) = \sum_{\tup \in \pt{\query, \db, \tup_1}} \mathbb{1}[{\exists \tup' ( \tup' \pmatch \pat \land \tup' \in \jtr(\jgraph, \pat) \land \tup \subseteq \tup'}]
%$$
$Pre(\dexpl) = \frac{TP}{TP+FP}$ , where $$TP = \sum_{\tup \in \pt{\query, \db, \tup_1}} \mathbb{1}[\tup \in \projection_{\att_{\ptlabel}} \matches \big(\pat,  \jtr(Q, \jgraph, \db, \tup) \big)]$$
$$FP =  \sum_{\tup \in \pt{\query, \db, \tup_2}}\mathbb{1}[ \tup \in \projection_{\att_{\ptlabel}}\matches \big(\pat, \jtr(Q, \jgraph, \db, \tup) \big) ]$$

where $\mathbb{1}[]$ is the indicator function, $\att_{\ptlabel}$ is the schema of the provenance table $\pt{\query, \db, \tup_1}$; the recall is defined as
$$
% Rec(\dexpl) = \sum_{\tup \in \pt{\query, \db, \tup_1}} \frac{\mid \matches \big(\pat, \selection_{\tup,  \pt{\query, \db, \tup_1}} \jtr(\jgraph, \pat) \big)\mid}{\mid {\selection_{\tup, \pt{\query, \db, \tup_1}} \jtr(\jgraph, \pat)} \mid}
Rec(\dexpl) = \sum_{\tup \in \pt{\query, \db, \tup_1}} \frac{\mid \matches \big(\pat,  \jtr(\jgraph, \db, \tup) \big)\mid}{\mid { \jtr(\jgraph, \db, \tup)} \mid}
$$

% where $\att^1$ and $\att^2$ are the schema of $\pt{\query, \db, \tup_1}}$ and $\pt{\query, \db, \tup_2}}$, and $\selection_{\tup, \att^i}$ is the selection on the join graph result choosing tuples whose $\pt{\query, \db, \tup_i}$ part is equal to $\tup$.

\end{Definition}
}

To ensure that this is the case, we
\BG{Now with the hindsight of the formal definitions reexplain the intro example}

\textbf{Quality measure of summarization patterns over all join graphs.~} \CL{This section is not implemented yet, the current framework only generates the Fscores, without considering the effects of the number of edges in the score}
Furthermore, we prefer explanations that are simpler, i.e., that have smaller join graphs. We incorporate these requirements into a quality measure for explanations, since using only \fscore\ may fail to reveal such simple but informative patterns. Similar to the widely-used weight function that considers the number of non-$\placeh$ values in the pattern in in prior data summarization works, we consider the number of edges in the schema join graph as the weight.

\begin{Definition}[Score Function]\label{def:score-function-all}
The score of an explanation $\sexpl = (\jgraph, \pat)$ is defined as
% $$Score(\sexpl) = \fscore(\sexpl) \times \frac{1}{1+e^{-\frac{B-|\jgraph.E|}{B-A}}}$$,
$$Score(\sexpl) = \fscore(\sexpl) \times \frac{B-|\jgraph.E|+1}{B-A+1}$$,
where $\jgraph.E$ denotes set of edges of the schema join graph, $A = \min_{\jgraph'\in \mathcal{E}} |\jgraph'.E|$, $B = \max_{\jgraph'\in \mathcal{E}} |\jgraph'.E|$, $\mathcal{E}$ is the set of of all candidate explanations.
\end{Definition}

\BG{Add formal problem definition: Given database D, schema graph, two-point or one-point question, generate top-k explanations for all join graphs (or subset thereof)}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/single_summary.tex <==
\section{Single-answer Summarization}

\begin{itemize}
    \item Search-problem, try out different joins and summarize join results optimize for globally best pattern
\end{itemize}

\begin{Definition}[Join-augmented Summarization Problem]
Given a database $\db$, a \termSchemaGraph for $\db$ $\sgraph$, a \abbrAggJoinQ $\query$, an output tuple $\tup$ of interest in the answer of $\query(\db)$, and a constant $\topk$, the join-augmented summarization problem $\JASP(\db, \sgraph, \query, \tup, \topk)$ is to find 
%a set of join trees  {\bf$ \jgraph$} and a set of patterns {\bf P} with the size of $K$ for  {\bf $\jgraph = \jjgraph$} such that those $K$ patterns have the highest $F_1(p)$ scores across all join trees for $Q$, $D$, $t$ and $G$.
a set $\explset$ consisting of $\topk$ explanations with the highest $F_1$ scores across all join trees for $Q$, $D$, $t$ and $G$.

\end{Definition}

%As motivated in our running example, if a user asks for explanations for a high/low outcome, we then find patterns by solving $\JASP(D, G, Q, t, \theta_{t, dir}(Prv(t)), K)$ where $\theta_{t, dir}$ is a filter on tuples in the provenance based on the aggregate value and the direction in the user question.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/solution_overview.tex <==
\section{Complexity and Solution Approach}
\label{sec:solution-overview}
\cut{
Note that even the problem we are solving in this work is \NPhard, because even
just finding patterns for a single $\jtr$ is \NPhard. \BG{add theorem to previous
  section or reference other papers whose results would imply that.}
  }

  First, we discuss the complexity of the optimization problems described in the previous section. Then we give an overview of the solutions in our work that utilizes a set of heuristic optimizations for each step in the complex process of join graph enumeration and mining top patterns that allow us to achieve reasonable performance without forsaking solution quality.
%\BG{This is vague, something more concrete we can say?}
\subsection{Complexity}\label{sec:complexity}
\textbf{Top-$k$ patterns with individual highest \abbrFs.~}
Finding top-$k$ patterns based on their individual scores has polynomial data complexity that considers fixed size of the schema and query \cite{Vardi82}. The provenance table and augmented provenance tables can be computed in polynomial time in the size of the data. Given a pattern, the matches can be evaluated in polynomial time and therefore, coverage, true/false positive and false negative, and precision/recall/\abbrF can be computed in polynomial time. If there are $p$ attributes in the augmented provenance table, the number of possible patterns is bounded by $O(n^p)$ (the number of distinct attribute values is bounded by $n$ = total number of tuples in all relations in the database, and each attribute can appear as don't care $*$ and with at most three comparison operators), so a naive approach of computing the top-$k$ patterns with the highest \abbrF values can be done in polynomial time in data complexity. However, this naive approach is not scalable for practical purposes and therefore we adopt a number of optimization heuristics to solve this problem as described in Section~\ref{sec:overview}.
\par
\textbf{Achieving a given combined \abbrF with a small patternset.~} This problem is computationally hard as shown below:
\begin{proposition}
Finding the smallest set $\patrnset$ of patterns given a fixed join graph achieving a given combined \abbrF is NP-hard in data complexity.
\end{proposition}
\begin{proof}
We give a reduction from the problem of finding a minimum vertex cover in a tri-partite graph, which is known to be NP-hard \cite{LlewellynTT93}. Given a tri-partite graph $G$ with partitions of vertices into $U, V, W$ and edges $E$ (no two vertices in the same partition can have a connecting edge), the goal is to decide if there is a subset $S \subseteq U \cup V \cup W$ of size $|S| \leq M$ such that for every edge in $E$, one of the two endpoints belongs to $S$. Suppose $n = |U| + |V| + |W|$ and $m = |E|$.
\par
Given such a graph $G$, we construct an instance of our problem as follows. There are two relations $R_1(A_1, A_E)$ and  $R_2(A_E, B_U, B_V, B_W)$ in the database $D$. For every edge $(u, v) \in E$ where $u \in U, v \in V$, we insert one tuple of the form $(1, E_{uv})$
%and one tuple of the form $(2, E_{uv})$
in $R_1$. We also insert one tuple of the form $(E_{uv}, u, v, W_{uv})$ in $R_2$. Similarly tuples of the form
$R_1(1, E_{vw})$ and $R_2(E_{vw}, U_{vw}, v, w)$ are inserted for edges $(v, w) \in E$ where $v \in V, w \in W$, and tuples of the form $R_1(1, E_{uw})$ and $R_2(E_{uw}, u, V_{uw}, w)$ are inserted for edges $(u, w) \in E$ where $u \in U, w \in W$. Finally, we insert $n$ tuples corresponding to the vertices $u \in U \cup V \cup W$ in $G$ to $(2, E_u)$ to $R_1$ and one tuple of the form $(E_u, u, V_u, W_u)$ to $R_2$. The query $Q$ is {\tt SELECT $A_1$, count(*) FROM $R_1$ GROUP BY $A_1$}, the results in $Q(R_1)$ are $t_1 = (1, m)$ and $t_2 = (2, n)$, and the user question asks to differentiate these two tuples.
\par
We consider the join graph $\jgraph$ where $R_1, R_2$ are joined on $R_1.A_E = R_2.A_E$, giving an augmented provenance table (APT). We claim that there is a vertex cover $S$ of size $\leq M$ in $G$ if and only if there is a set of pattern $\patrnset$ in $D$ for this join graph $\jgraph$ with size $|\patrnset| \leq n$ giving  $\fscore(\patrnset, \jgraph, t_1, t_2) \geq \frac{2}{2m + M}$.
\par
(only if) Suppose there is a vertex cover $S$ in $G$ of size $\leq M$. For every $u \in U \cap S$, we include the pattern $(A_U: u, =)$  in $\patrnset$ (i.e., a tuple $t$ in the APT will match if $t.A_U = u$); similarly for $v \in V \cap S$, we include the pattern $(A_V: v, =)$ and for $w \in W \cap S$, we include the pattern $(A_W: w, =)$ in $\patrnset$. Since, $S$ is a vertex cover, all $m$ tuples in the provenance of $t_1$ corresponding to the edges are covered by  $\patrnset$. Further, the tuples in the provenance of $t_2$ corresponding to the vertices in $S$ are covered. Hence, $\ITP(\sexpl, \jgraph, \tup_1) = m$, $\IFN(\sexpl, \jgraph, \tup_1) = 0$, $\IFP(\sexpl, \jgraph, \tup_1, \tup_2) \leq M$. Therefore, $\Rec = \frac{m}{m + 0}$, $\Prec \geq \frac{m}{m + M}$, $\fscore \geq \frac{2m}{2m + M}$.
\par
(if) Consider a pattern set $\patrnset$  giving $\fscore(\patrnset, \jgraph, t_1, t_2) \geq \frac{2m}{2m + M}$ of size $|\patrnset| \leq n$. Since the group-by attributes cannot appear in a pattern, any pattern in $\patrnset$ can only have attributes $A_E, B_U, B_V, B_W$. First, we argue that any pattern in $\patrnset$ without loss of generality (i) either can be assumed to be of the form $(A_U: u, =)$, $(A_V: V, =)$, or $(A_W: w, =)$, i.e. except exactly one of $A_U, A_V, A_W$ taking a value of a vertex from $G$, the rest of the attributes would be $*$, (ii) or it uniquely covers an edge tuple $R_1(1, E_{u, v})$, $(u, v) \in E$. Suppose in $\patrnset$ there is a pattern $\pat$ involving any other attribute or multiple attributes. Clearly, if the pattern involves attribute values of the form $U_u, V_u, W_u$, then they only lead to false negatives without any true positives and can be removed from $\patrnset$ without reducing the \abbrF values.
\par
If a pattern $\pat$ includes attribute values $E_{uv}, U_{uv}, V_{uv}, W_{uv}$ for $(u, v) \in E$, or two of the vertices in these edge tuples, e.g., $(A_U: u, =) \wedge (A_V: v, =)$, then it matches exactly one edge tuple in the provenance of $t_1$ (here $(1, E_{uv})$), and no vertex tuples in the provenance of $t_2$ of the form $(2, E_u)$. If such a pattern is encountered in $\patrnset$, we check if the pattern $(A_U: u, =)$ or $(A_V: v, =)$ is already included in $\patrnset$. If yes, we simply discard $\pat$ as $R_1(1, E_{uv})$ is already covered in $\patrnset$. If not, we check replacing  it with another pattern $\pat' = (A_U: u, =)$ or $\pat' = (A_V: v, =)$ covers $L \geq 1$ new edge tuples in the provenance of $t_1$ (at least one new tuple is covered in the provenance). If yes, then we replace $\pat$ with such  $\pat' = (A_U: u, =)$ or $\pat' = (A_V: v, =)$ forming a new patternset $\patrnset'$. Suppose the old true positive and false positive for $\patrnset$ are $tp_1, fp_1$ respectively. Then the new true and false positive values are $tp_2 = tp_1 + L$, and $fp_2 = fp_1 + 1$, as exactly one of $R_1(2, E_u)$ or $R_1(2, E_v)$ in the provenance of $t_2$ is now covered. Both old and new false negatives are zero. Old recall is $R1 = \frac{tp_1}{m}$, precision is $P1 = \frac{tp_1}{tp_1 + fp_1}$, and \abbrF is $F1 = \frac{2tp_1}{m + tp_1 + fp_1}$. New recall is $R2 = \frac{tp_1 + L}{m}$, precision is $P2 = \frac{tp_1 + L}{tp_1 + L + fp_1 + 1}$, and \abbrF is $F2 = \frac{2(tp_1 + L)}{m + tp_1 + L + fp_1 +1}$. Now $F1 \leq F2$, since $tp_1 (m + tp_1 + L + fp_1 +1) - (tp_1 + L)(m + tp_1 + fp_1) = tp_1 - Lm - fp_1L$ $\leq -m(L-1) - fp_1 L \leq 0$ since $L \geq 1$ and $tp_1 \leq m$. Hence replacing $\patrnset$ with $\patrnset'$ does not reduce the \abbrF.
\par
After repeating the above process until no more replacement can be made, we will be left with a patternset $\patrnset'$ (i) either patterns of forms $(A_U: u, =)$, $(A_V: V, =)$, or $(A_W: w, =)$, or (ii) patterns involving at least one of $A_{uv}, U_{uv}, V_{uv}, W_{uv}$ or involving both of $u, v$ for $(u, v) \in E$, such that exactly one tuple $R_1(1, E_{uv})$ is covered by such pattern.
We claim that all tuples $R_1(1, E_{uv})$ in the provenance of $t_1$ are covered by $\patrnset'$, otherwise if such an edge tuple is uncovered, we include either $(A_U: u, =)$ or $(A_V: V, =)$ and repeat the above argument to show that the \abbrF is not decreased.
For patterns of form (i), we include the corresponding vertex in $G$ to a set $S$. For patterns of the form (ii), we include any one of the vertices $u$ or $v$ to $S$. Suppose $|S| = M'$, with $M_1'$ vertices coming from (i) and $M_2'$ vertices coming from (ii). Then the recall, precision, and \abbrF of this new pattern set is $R = \frac{m}{m + 0}, P = \frac{m}{m + M_1'}, F = \frac{2m}{2m + M_1'} \geq \frac{2m}{2m + M}$. \red{INcomplete}
\end{proof}
\subsection{Solution Overview}\label{sec:overview}
To generate explanations we have to enumerate the join graphs induced by the
provenance table and the schema graph provided as part of the input. For each
such join graph $\jgraph$ we then have to compute the corresponding \termAPT and
find the top-$k$ patterns (the patterns with the greatest scores). A major
challenge is the size of the search space. The number of join graphs of a given
size (number of edges) is exponential in the size. Furthermore, the number of
pattern candidates for a given \abbrAPT $\jtr$ is exponential in the number of
attributes of $\jtr$.

The optimizations we employ reduce the size of the search space as well as
reduce the cost of individual operations. We give a brief overview here and will
discuss each optimization in more detail in~\Cref{sec:algo}
and~\Cref{sec:join-graph-enumeration}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Pruning Join Graph Candidates}
%
Even though we require that a join graph consist of a single connected
component, some \abbrAPTs may still be large because not all possible join
conditions between tables in the join graph that are permitted by a schema graph
have to be included. For instance, if a person has a work as well as a home
address, then join graphs are not required to join on both home and work
address. This is sensible, because otherwise we would only consider persons that
live and work at the same address. However, in some cases this can lead to
redundancy that can be avoided. Specifically, if not all primary key attributes
of a table are joined with other tables in the join graph. For instance,
consider the provenance table of a query that joins the Game,
LineupPerGameStats, and LineupPlayer tables. Furthermore, consider a join graph
that joins this provenance table with PlayerGameScoring on the primary key of
the game table (year, month, day, home).  \BG{Furthermore, even join graphs
  created based on a schema graph that only allows key-foreignkey joins may
  contain redundant (indirect) self-joins where tuples are only joined with
  themselves. As a trivial example, consider a schema $author(name)$,
  $author-publication(author,title)$ storing who has published which paper and a
  schema graph with a single join condition
  $author.name = author-publication.author$. One valid join graph for this
  schema graph is joining the author table with author-publication and then
  author-publication with another copy of author. Each tuple in the \abbrAPT
  corresponding to this join graph contains the same author twice. While in this
  example it would be easy to detect the redundancy, in general this is not the
  case.  INSERT COMPLEX EXAMPLE HERE.  We conjecture that it may be possible to
  detect such cases by reasoning about equality-generating dependencies that
  hold over join results implied by keys and inclusion dependencies (foreign
  keys). However, this is beyond the scope of this paper. We employ a practical
  alternative: we use a DBMS to estimate the cost of the query generating an
  \abbrAPT and skip generating the \abbrAPT when this cost is higher than a
  configurable threshold.  }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Filtering and Clustering \abbrAPT Attributes}
%
As mentioned above, the number of candidate patterns is exponential in the
number of attributes of the \abbrAPT for which we are generating patterns. We
employ two methods to reduce the number of attributes to be considered for
pattern generation: (i) we determine the importance of each attribute in the
\abbrAPT in distinguishing between augmented provenance or rows that do not
belong to the provenance. Attributes of low importance are excluded from pattern
generation since they are unlikely to produce explanations of high quality; and
(ii) we cluster attributes based on pair-wise correlations between
attributes. The intuition is that strongly correlated attributes lead to
redundancy in patterns. For instance, consider a functional dependency
$zipcode \to city$, adding \textit{city} to a pattern that already contains
\textit{zipcode} is redundant since the set of matches for the extended pattern
is exactly the same as for the pattern that only uses attribute
\textit{city}. We enforce that each pattern only contains a single attribute
from each cluster and present the clusters to the user as additional auxiliary
information. In addition to significantly reducing the number of patterns to be
considered, this optimization reduces the amount of redundancy within patterns
and often leads to more diverse sets of top-k patterns, because we avoid the
situation where multiple redundant variants of one pattern dominate the result.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Pattern Candidate Generation}
%
We employ the LCA algorithm from~\cite{DBLP:journals/pvldb/GebalyAGKS14} to
compute patterns over solely consist of equality comparisons over categorical
attributes by generalizing pairs of tuples from a sample drawn from an
\abbrAPT. Patterns with a recall above a configurable threshold are then
extended by adding inequality conditions on numeric attributes. The rationale
for this approach is that adding additional comparisons to a pattern can only
reduce the patterns recall and may or may not improve the patterns precision. By
pre-filtering more general patterns (less comparisons) based on their recall, we
can avoid generating many pattern candidates that are guaranteed to have low
recall since they extend patterns with low recall.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Using Sampling for Quality Score Estimation}
%
One major cost factor of determining the top-k patterns for an \abbrAPT is
calculating precision and recall to determine the score of a pattern by joining
the pattern with the \abbrAPT to determine all matches for the pattern. Similar
to past work on pattern-based
explanations~\cite{DBLP:journals/pvldb/GebalyAGKS14,LL20}, we determine matches
over a sample of the data and estimate precision and recall over this sample.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/user-study-tech.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
    \centering
    \small
    \begin{tabular}{c|p{25em}|p{25em}}

& \textbf{Provenance-based Explanations} & \textbf{\oursys{}}\\\midrule
\multirow{2}{*}{Expl1} &
In season 2015-16, among the games GSW won, they were the visiting team and they scored more than 104 points in 28 games.&
In 2015-16 season, the number of games with GSW player Stephen Curry's minutes $< 38$ and usage $> 25$ is 59 out of 73 games GSW won. \\
& In season 2012-13, among the games GSW won, they were the visiting team and they scored more than 104 points in 10 games. &
In 2012-13 season, the number of games with GSW player Stephen Curry's minutes $< 38$ and usage $> 25$ is 12 out of 47 games GSW won.	\\\midrule
\multirow{2}{*}{Expl2} &
In 2015-16 season, 73 out of 73 games GSW won are regular season games. & In 2015-16 season, the number of games with GSW player Draymond Green's minutes>15 is 73 out of 73 games GSW won.\\
& In 2012-13 season, 47 out of 47 games GSW won are regular season games. & In 2012-13 season, the number of games with GSW player Draymond Green's minutes>15 is 15 out of 47 games GSW won. \\\midrule
\multirow{2}{*}{Expl3} &
In 2015-16 season, Among the games GSW won,they were the visiting team and they scored more than 98 points and had more than 101 possessions in 17 games. & In 2015-16 season, Jarrett Jack played in 0 out of 73 games GSW won.\\
& In 2012-13 season, Among the games GSW won,they were the visiting team and they scored more than 98 points and had more than 101 possessions in 0 games. & In 2012-13 season, Jarrett Jack played in 47 out of 47 games GSW won.	\\\midrule
\multirow{2}{*}{Expl4} &
In 2015-16 season, GSW scored more than 104 points in each of 64 out of 73 games GSW won. & In 2015-16 season, GSW team had three\_pct $> 35\%$ and points $> 112$ in each of 39 out of 73 games GSW won.\\
& In 2012-13 season, GSW scored more than 104 points in each of 24 out of 47 games GSW won. & In 2012-13 season, GSW team had three\_pct $> 35\%$ and points $> 112$ in each of 9 out of 47 games GSW won.
\\\midrule
\multirow{2}{*}{Expl5} &
In 2015-16 season, the home teams (could be GSW or the opponent) scored less than 106 points and had less than 101 possessions in each of 29 out of 73 games GSW won.
& In 2015-16 season, GSW had fg\_three\_pct $> 48\%$ and points $> 112$ and rebounds $> 51$ in 5 out of 73 games GSW won.\\
& In 2012-13 season, the home teams (could be GSW or the opponent) scored less than 106 points and had less than 101 possessions in each of 40 out of 47 games GSW won. & In 2012-13 season, GSW had fg\_three\_pct $> 48\%$ and points $> 112$ and rebounds $> 51$ in 2 out of 47 games GSW won.
\\\bottomrule
    \end{tabular}
    \caption{Explanations used in the user study}
    \label{tab:user_study_expls}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\revm{
\section*{User Study}\label{sec:user-study-tech}
We have conducted a user study to evaluate % (1) the utility of explanations produced by \oursys{} and (2) the effectiveness our  quality metric. Furthermore, we wanted to evaluate how explanations produced by \oursys{} compare against explanations generated based on provenance along.
% Specifically, we want to know:
(S1) whether
\oursys{} provides meaningful and informative explanations in addition to explanations that only come from the provenance; (S2) whether
the quality metric used in \oursys{} is consistent with users' preference; and also (S3) the effect of domain knowledge and/or familiarity with database queries (if any) on the usefulness of these explanations. % \oursys{} to a user.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\revm{
\subsection*{User Study Setup}\label{sec:study-setup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mypar{Dataset and queries}.
We use a subset of the NBA dataset that contains 11 tables; we combine all player game statistics into one single table for simplicity. Reconsider query $\query_1$ introduced in \Cref{exp:GSW} which counts the number of winning games per season for GSW.
In the study, we use query $\query'_1$ which is an adaption of $\query$ for the simplified schema:
}
\begin{lstlisting}[escapeinside=!!]
!$\query'_1=$!
   SELECT s.season_name, COUNT(*) AS win
   FROM team t, game g, season s
   WHERE t.team_id = g.winner_id
     AND g.season_id = s.season_id AND t.team = 'GSW'
   GROUP BY s.season_name
\end{lstlisting}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\revm{\mypar{Participants.} We conducted a study with 20 participants - all of them are
graduate students studying in different areas of computer science,
and 13 of them have some prior experience with SQL. We did ask these participants to explore the dataset and manually find explanations for an outcome using SQL before asking them to rate explanations produced by our approach. For those who unfamiliar with SQL, we skipped the exploration phase. Out of the 20 participants, 5 were NBA fans, 9 (including the 5 fans) were familiar with basketball, and 10 had no prior domain knowledge.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \mypar{Tasks.}
%
\revm{Each participant was asked to find and/or evaluate explanations for the user question $\uquestion_1$ from \Cref{exp:GSW}: ``\emph{Why did $\abbrGSW$ win 73 games in season $2015 \mbox{-} 16$ compared to 47 games in $2012 \mbox{-} 13$.}'' based on the result of query $\query'_1$.  % over the NBA dataset.
  We selected five explanations for users to evaluate from each explanation method (\textit{provenance-based} and \textit{\oursys{}}). The five explanations for the provenance-based method were the top 5 explanations with the highest \abbrF produced by this method. Because the top explanations by \oursys{} tend to have higher \abbrFs than the ones produced by the provenance-based method (see Table~\ref{tab:avg_score}), we added one with low \abbrF (Expl5 of \oursys{} in \Cref{tab:avg_score}).
%\sudeepa{what does Expl 5 mean?}
% with low \abbrF.
By covering a wider range of \abbrF values, we aimed to find out for (S2) above (1) whether the users can distinguish high score explanations and low score explanations, and (2) whether the users agree with our quality measures on ranking the ``good'' explanations.
 }

\revm{
The study consisted of five phases: (a) in the \emph{background information collection phase} we asked the participants whether they are familiar with SQL and basketball in general, Furthermore, we asked whether they are NBA fans; (b) in the \emph{introduction phase} we presented to the participants basic background knowledge on basketball game and the NBA, described the schema of the dataset using an ER-diagram, and explained the query and the question for which explanations should be generated; (c) in the \emph{exploration phase} we gave the participants 20 minutes to explore the NBA dataset and seek for explanations to the given question;
(d) we then asked participants to fill \emph{a survey to obtain users ratings} (scale of 1 to 5) for each of the five explanations generated by the provenance-based method and five explanations generated by \oursys{} (half of the participants were shown explanations produced by the provenance-based method first while the other half were shown the  explanations produced by \oursys{} first); and (e) in the \emph{assessment phase} we asked participants which set of explanations made more sense (provenance-based or \oursys{}) and which set of explanations provided new insights that helped them to answer the question (provenance-based, \oursys{}, or both), and if they had any suggestions on what other information would be useful for finding explanations for the questions.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\revm{
\subsection*{User Study Results}\label{sec:study-results}
Overall, the responses were positive: 16 out of 20 participants agree that explanations by \oursys{} make more sense to them and seeing explanations by \oursys{} in advance will help them finding new explanations that they did not think about before.
}

% Method A	Exp1	Exp2 	Exp3 	Exp4	Exp5
% f1	0.69	0.56	0.38	0.8	0.4
% recall	0.383	1	0.23	0.87	0.4
% precision	0.74	0.61	1	0.73	0.4





% Method B	Exp1	Exp2 	Exp3 	Exp4	Exp5
% 	0.82	0.91	1	0.64	0.13
% recall	0.83	1	1	0.53	0.07
% precision	0.81	0.83	1	0.81	0.7

%\setlength{\tabcolsep}{3pt}
\begin{table}[!ht]

\caption{\revm{\small Average ratings for each explanation by users with different expertise and the measures for each explanation by \oursys{}}} \label{tab:avg_score}
\small
\resizebox{0.48\textwidth}{!}{
%\revmcolor
\begin{tabular}{c|ccccc|ccccc}\toprule
                 & \multicolumn{5}{c|}{Provenance-based} & \multicolumn{5}{c}{\oursys{}}                                         \\
                 & Expl1                                 & Expl2 & Expl3 & Expl4 & Expl5 & Expl1 & Expl2 & Expl3 & Expl4 & Expl5 \\ \midrule
%Rank by \abbrF & 2                                     & 3     & 5     & 1     & 4     & 2     & 1     & Expl3 & Expl4 & Expl5 \\ \midrule
All	users        & 3.150                                 & 1.450 & 3.950 & 3.600 & 2.750 & 3.600 & 3.800 & 2.350 & 3.950 & 2.300 \\
Stdev            & 1.040                                 & 0.999 & 0.759 & 1.095 & 1.410 & 0.883 & 1.196 & 1.424 & 0.999 & 1.174 \\ \midrule
SQL: Yes         & 3.286                                 & 1.643 & 4.000 & 3.786 & 2.929 & 3.571 & 4.143 & 2.571 & 4.000 & 2.429 \\
SQL: No          & 2.833                                 & 1.000 & 3.833 & 3.167 & 2.333 & 3.667 & 3.000 & 1.833 & 3.833 & 2.000 \\
Basketball: Yes  & 3.667                                 & 1.778 & 4.222 & 3.778 & 2.889 & 3.889 & 3.444 & 2.444 & 4.333 & 2.444 \\
Basketball: No   & 2.727                                 & 1.182 & 3.727 & 3.455 & 2.636 & 3.364 & 4.091 & 2.273 & 3.636 & 2.182 \\
NBA: Yes         & 3.400                                 & 1.800 & 3.800 & 3.600 & 2.800 & 3.800 & 3.800 & 2.800 & 4.200 & 2.600 \\
NBA: No          & 3.067                                 & 1.333 & 4.000 & 3.600 & 2.733 & 3.533 & 3.800 & 2.200 & 3.867 & 2.200 \\\midrule
\abbrF          & 0.69                                  & 0.56  & 0.38  & 0.8   & 0.4   & 0.82  & 0.91  & 1     & 0.64  & 0.13  \\
recall           & 0.38                                  & 1     & 0.23  & 0.87  & 0.4   & 0.81  & 1     & 0.99  & 0.53  & 0.07  \\
precision        & 0.74                                  & 0.61  & 1     & 0.73  & 0.4   & 0.83  & 0.83  & 0.99  & 0.81  & 0.7   \\\bottomrule
\end{tabular}}
\end{table}

\revm{
Table~\ref{tab:avg_score} shows the average user ratings and quality measures for each explanation used in the study.  Ratings are between 1 and 5, and precision, recall, and \abbrF between 0 and 1. From Table~\ref{tab:avg_score}, for (S1), we see that the average ratings of the top-1 explanation are the same for both methods, while for the next two explanations \oursys{} has higher average ratings (3.95 vs 3.95, 3.8 vs 3.6, 3.6 vs 3.15). The margin becomes bigger for user who are familiar with the NBA domain (4.2 vs 3.8, 3.8 vs 3.6, 3.8 vs 3.4). }

\revm{
To answer (S2), we compare the user ratings with our quality measures. We find that explanations with high user ratings (Expl 3 and 4 of the Provenance-based method, Expl 1, 2, 4 of \oursys{}) are highly correlated to high \abbrF and precision, with  one exception, Expl 3 of \oursys{}, which is also the most controversial one among the users as indicated by having the greatest standard deviation. Next, we evaluate the ranking results by our different quality measures. For pairwise ranking error, we use Kendall-Tau rank distance~\cite{kendall1938new} that counts the number of reverse pairs in two ranking lists. }
\revm{
First, we regard user ratings as the ground truth for ranking the explanations. We compare ranking based on our quality measures with both ranking by average and individual user ratings.
As shown in \Cref{tab:ranking}, we see that ranking by precision gives the lowest pairwise ranking error for the provenance-based method, while ranking on \abbrF is close to precision for our method. As mentioned before, if we ignore the most controversial explanation, the pairwise error is reduced by more than half. }
%Moreover, ranking without ties is sometimes too strict, for example, for explanations by \oursys{}, putting Expl2 (rated 3.8) before Expl4 (rated 3.95) is counted as one reverse pair, which is the same as putting Expl5 (rated 2.3) before Expl4.
\revm{Moreover, as the user ratings can have ties, we further allow ties in the ranking lists if the measures are close enough. The results for such coarse-grained ranking as shown in \Cref{tab:ranking} reinforces that our quality measures are close to users' ranking results, especially after skipping controversial ones.}
%and the most controversial explanation largely affects the ranking result.

\revm{
We also evaluate the effectiveness of our quality measures using normalized discounted cumulative gain (NDCG)~\cite{jarvelin2002cumulated}, which is often used in information retrieval for evaluating recommendation and searching algorithms.
$NDCG_n = \frac{DCG_n}{IDCG_n}$, where $DCG_n$ is the weighted sum of graded relevance of top $n$ ranked items $DCG_n = \sum_{i}^{n}\frac{2^{rel_i}}{\log_2(i+1)}$, and $IDCG_n$, the ideal $DCG$ of the top $n$ ranked items, is the  $DCG$ score among all rankings of these items. $NDCG$ is always a value between 0 and 1.
By treating the rating of each explanation as the graded relevance, we compute $NDCG_n$ ($n=5$ for all explanations while $n=4$ for dropping the most controversial explanation) for each user to evaluate our quality measures. As shown in \Cref{tab:ranking}, the $NDCG_n$ of all three measures for \oursys{} reaches 0.9 for all cases and is even 0.95 after dropping the most controversial explanation; the $NDCG_n$ of precision for the provenance-based method is obviously higher than \abbrF and recall. Note that $NDCG_n$ is higher among users who are familiar with the NBA basketball domain in most cases.
}

\begin{table}[t]
% \caption{\small Ranking lists for two sets of explanations by two methods.} \label{tab:ranking}
% \small
% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|ccccc|ccccc}\toprule
% & \multicolumn{5}{c|}{Explanation Tables} & \multicolumn{5}{c}{\oursys{}}    \\
% 0& Expl1 & Expl2 &Expl3 &  Expl4 &Expl5 & Expl1 & Expl2 &Expl3 &  Expl4 &Expl5  \\ \midrule
% User ratings & 3 & 5 & 1 & 2 & 4 & 3 & 2 & 4 & 1 & 5\\\midrule
% \abbrF & 2 & 3 & 5 & 1 & 4 & 3 & 2 & 1 & 4 & 5\\
% recall & 4 & 1 & 5 & 2 & 3 & 3 & 1 & 2 & 4 & 5\\
% precision &  2 & 4 & 1 & 3 & 5 & 3 & 2 & 1 & 4 & 5 \\\bottomrule
% \end{tabular}
% }
\caption{\revm{Measures of ranking quality. \emph{All} denotes all five explanations and \emph{Drop One} indicates dropping the explanation with the biggest standard deviation}.} \label{tab:ranking}
%\small
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|cc|cc}\toprule
\multicolumn{3}{c}{\multirow{2}{*}{}} & Explanation Tables & \oursys{}  \\
 \multicolumn{3}{c}{}&  All / Drop One & All / Drop One \\ \midrule
\multirow{3}{5em}{Kendall tau rank distance} &\multirow{3}{10em}{Ranking by avg. user ratings} & \abbrF & 5 / 3 & 5 / 2\\
% recall & 8 / 5 & 4 / 2 \\
% precision &  2 / 1 & 4 / 1 \\\bottomrule
& &recall & 8 / 5 & 5 / 2 \\
& &precision &  2 / 1 & 5 / 2 \\\midrule
\multirow{12}{5em}{Avg. Kendall tau rank distance} & \multirow{3}{10em}{All users, fine-grained} & \abbrF & 3.95 / 2.2 & 3.9 / 1.4\\
& &recall & 5.9 / 3.85 & 3.3 / 1.4 \\
& &precision &  2.2 / 0.95 & 3.9 / 1.4\\
% \multirow{}{7em}{Avg. Kendall tau rank distance} &
& \multirow{3}{10em}{Users with domain knowledge, fine-grained} & \abbrF & 3.6 / 2.0 & 3.2 / 1.8\\
& &recall & 5.2 / 3.2 & 3.8 / 1.8 \\
& &precision &  2.2 / 1.2 & 4.2 / 1.8\\
\cline{2-5}
 & \multirow{3}{10em}{All users, coarse-grained} & \abbrF & 3.3 / 2.15 & 3.2 / 1.4\\
& &recall & 4.45 / 2.4 & 3.2 / 1.4 \\
& &precision &  1.1 / 0.55 & 2.75 / 0.25\\
& \multirow{3}{10em}{Users with domain knowledge, coarse-grained} & \abbrF & 3.8 / 1.8 & 3.6 / 1.8\\
& &recall & 4.2 / 2.2 & 3.6 / 1.8 \\
& &precision &  1.2 / 0.8 & 2.8 / 0.4\\\midrule
\multirow{12}{5em}{Avg. $NDCG_n$} & \multirow{3}{10em}{All users, fine-grained} & \abbrF & 0.875 / 0.882 & 0.901 / 0.955\\
& &recall & 0.844 / 0.852 & 0.901 / 0.955 \\
& &precision &  0.933 / 0.965 & 0.901 / 0.955\\\cline{2-5}
 & \multirow{3}{10em}{Users with domain knowledge, fine-grained} & \abbrF & 0.897 / 0.901 & 0.903 / 0.954\\
& &recall & 0.862 / 0.878 & 0.903 / 0.954 \\
& &precision &  0.953 / 0.977 & 0.903 / 0.954 \\
\cline{2-5}
& \multirow{3}{10em}{all users, coarse-grained} & \abbrF & 0.904 / 0.844 & 0.890 / 0.910\\
& &recall & 0.847 / 0.791 & 0.890 / 0.910 \\
& &precision &  0.963 / 0.899 & 0.867 / 0.917 \\\cline{2-5}
& \multirow{3}{10em}{Users with domain knowledge, coarse-grained} & \abbrF & 0.925 / 0.873 & 0.901 / 0.913\\
& &recall & 0.870 / 0.824 & 0.901 / 0.913 \\
& &precision &  0.969 / 0.913 & 0.886 / 0.924 \\
% \multirow{12}{5em}{Avg. $NDCG_4$} & \multirow{3}{10em}{All users, fine-grained} & \abbrF & 0.799 / 0.882 & 0.824 / 0.955\\
% & &recall & 0.725 / 0.852 & 0.824 / 0.955 \\
% & &precision &  0.894 / 0.965 & 0.824 / 0.955\\\cline{2-5}
%  & \multirow{3}{10em}{Users with domain knowledge, fine-grained} & \abbrF & 0.821 / 0.901 & 0.850 / 0.954\\
% & &recall & 0.755 / 0.878 & 0.850 / 0.954 \\
% & &precision &  0.915 / 0.977 & 0.850 / 0.954 \\
% \cline{2-5}
% & \multirow{3}{10em}{all users, coarse-grained} & \abbrF & 0.815 / 0.844 & 0.823 / 0.910\\
% & &recall & 0.747 / 0.791 & 0.823 / 0.910 \\
% & &precision &  0.930 / 0.899 & 0.833 / 0.917 \\\cline{2-5}
% & \multirow{3}{10em}{Users with domain knowledge, coarse-grained} & \abbrF & 0.848 / 0.873 & 0.847 / 0.913\\
% & &recall & 0.777 / 0.824 & 0.847 / 0.913 \\
% & &precision &  0.938 / 0.913 & 0.863 / 0.924 \\
\bottomrule
\end{tabular}}
\end{table}
%\scream{Need to add more ranking result and analysis.}
\noindent\revm{\textbf{Takeaways.} The main findings are: (1) the majority (16/20) of participants preferred our method, thanks to the new information provided by tables not used in the query; (2) our quality measures are consistent with users' preference; (3) for both methods, there can be top explanations rated low by users, which is as expected because we did not use causal analysis, and validating such explanations may be subjective and depend on domain expertise; and (4) users with domain knowledge had an even stronger preference for our method than users without domain knowledge.}

\revm{
Finally, it is also worth noting that the explanations and suggestions by users support the motivation of \oursys{}. For example, one user found that
\textit{"the total possessions of season 2015-16 is much higher than that of 2012-13.''} before s/he saw the explanations by \oursys{}. Another user suggested to use health information of the players in explanation. \oursys{} would be able to find such explanations after acquiring the data and joining the corresponding tables with the provenance.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../techreport"
%%% End:

